Generating Object Stamps

We present an algorithm to generate diverse foreground objects and composite them into background images using a GAN architecture. Given an object class, a user-provided bounding box, and a background image, we first use a mask generator to create an object shape, and then use a texture generator to fill the mask such that the texture integrates with the background. By separating the problem of object insertion into these two stages, we show that our model allows us to improve the realism of diverse object generation that also agrees with the provided background image. Our results on the challenging COCO dataset show improved overall quality and diversity compared to state-of-the-art object insertion approaches.

==> src/1-intro.tex <==
\vspace{-0.3cm}
\section{Introduction}

\vspace{-0.05cm}
Compositing objects into images is a common editing task. 
Given a database of images of a target object class and a specific background image, the task typically proceeds in three steps: 
1) Find an instance of the object in a suitable pose and under similar lighting to the background image; 
2) define the location and size of the object in the background image; and 
3) composite the object onto the background in a visually-consistent way.
Often this process can be cumbersome, and requires time and skill.

Our goal is to reduce the burdens of steps 1 and 3 to create a simple user interface for object compositing.
We begin with a database of images with object masks. 
Importantly, one requirement of our method is that it must work on images taken `in the wild', where objects have varied shapes, backgrounds, are not centered and scaled within the image, and can exist in multiple instances per image sometimes under significant occlusion.
We wish to learn how to represent the object class' appearance variation, and how to match the appearance with background scenes. 
This would let the user generate an object by simply dragging a bounding box over novel background images, and then by sampling multiple shapes and textures from the learned space of the object class.

\vspace{-0.25cm}
\paragraph{Motivation:} 
This problem is challenging as it requires understanding both the object class' diversity in appearance and how that appearance changes with the rest of the scene, \eg, how object appearance changes under scene lighting. 
Existing whole-image synthesis methods, such as conditional generative adversarial networks (cGANs), are at odds with our application scenario of placing objects against a \emph{specific} background. 
Further, whole-image methods can `cheat' at foreground generation by altering the background to satisfy the discriminator (\eg changing green grass to brown savanna when mapping from horse to zebra), which reduces translation quality.
Another option is to simultaneously generate object shape and texture, and paste the result into a specific background. 
However, doing so has several limitations.
For one, it prohibits the disentanglement of shape and texture, which is a useful interaction tool.
Second, the discriminator's ability to verify realism is overwhelmingly driven by texture~\cite{Geirhos2018}, which allows the generator to explore \emph{implausible shapes} to satisfy the discriminator.

% \ms{When reading this, I got confused. I didn't see the worlds ``diversity" or "lighting" anywhere. I think this paragraph would be made more clear if it went more like ``Whole image methods cheat by altering the target background, reducing emphasis on foreground generation and inhibiting their ability to match the object texture to the background rather than vice-versa.}

\begin{figure*}[t]
    \centering
    \includegraphics[clip,width=\linewidth]{figures_cvpr/Main.pdf}
    % \includegraphics[clip,width=0.495\linewidth]{figures_cvpr/Shape.pdf}
    % \includegraphics[clip,width=0.495\linewidth]{figures_cvpr/Texture.pdf}
    \caption{\emph{Overview of our image generation pipeline.} 
    Given an input image $i$, a bounding box is cut out to create $i_b$, and this is then fed into the mask generator $G_M$. $G_M$ creates a plausible object mask from the desired category (in this case, zebra). 
    Our texture generator then fills in the mask to produce a final composited image, while a texture discriminator ensure image realism.}
    \label{fig:architecture}
    \vspace{-0.25cm}
\end{figure*}

\vspace{-0.25cm}
\paragraph{Our approach:} Inspired by curriculum learning approaches, we decompose the generation process into two steps. 
First, we synthesize foreground masks (representing the shape of the object) conditioned on both a specific background image and user specified bounding box.
Next, we generate realistic texture within the mask via \emph{conditioning on the shape mask and background image}. 
This allows us to fix the shape while varying the texture (or vice versa), and allows us to explicitly enforce the realism of the shape and texture with separate discriminators.
%
% Both steps are jointly trained end-to-end, so that the shape generation is also aware of texture generation that follows.
%Specifically, we first learn to generate object masks conditioned on both a specific background image and a user specified bounding box. This step generates the shape of an object given where the object should go in that image.
%Next, we learn to generate object textures conditioned on the generated object mask and the background image.
At each stage, we inject randomness expressed by a latent random variable, which allows the generation of multiple shape masks and textures given the same bounding box coordinates.
%This randomness is injected via adaptive instance normalization layers and enforced via set reconstruction losses (Sec.~\ref{sec:Method}).
%Our approach can be trained from any dataset which includes mask annotations, as masks provide both samples of real object shapes, as well as a derived bounding box.
% In addition, we present a novel training scheme which handles real and fake samples differently during training. This enables us to train with images that have objects in them (e.g., from a semantic segmentation dataset) while at test time we can create object stamps on any image, whether it contains existing instances or not. 

We demonstrate our method trained on images and segmentation masks ``in-the-wild'' from COCO~\cite{MSCOCO2014}.
%which is a challenging dataset for GAN image synthesis, 
Recent work on the related task of image-to-image translation has shown that methods fail when trained on COCO images due to the large variation in the pose and appearance of objects and backgrounds~\cite{wu2019transgaga}.
%\ms{Maybe we can mention this earlier, along with the discussion of 'in-the-wild' images? Also, we can cite that SOTA GANs fail on this dataset. }
However, by splitting the problem into shape and texture generation, and leveraging masks to isolate foreground objects, we show that our method can generate plausible results despite the dataset variance. 
By disentangling shape from texture, our method can be used for three editing applications: generating an object with both new shape and texture and compositing it with a background image (`object stamps'), changing the texture of an existing object within an image (`object retexturing'), and adding objects with an existing shape into a new background image (`object insertion').

We compare our approach with solutions which synthesize a whole image at once, and well as state-of-the-art approaches that separate foreground and background generation~\cite{HierarchicalSemanticImageManpulation,finegan}. On the challenging COCO dataset with high variance, we found that existing approaches can mode collapse during training. However, our method is more robust: our curriculum learning strategy is easier to train than on both tasks jointly given a fixed parameter and data budget, and produces higher-quality mask shapes and textures than compared methods.
% \ow{We demonstrate the robustness of our method by applying it to a challenging ``in-the-wild'' dataset (COCO), and show that we found due to the variance in the data, existing approaches often collapse completely during training.}
%\ms{Can we mention the other approaches might even mode collapse? I think we might be able to make even stronger claims here about how our algorithm can handle complex shapes, now that FineGAN has collapsed.}
%In summary, our work suggests that a simpler compositing interface is possible by learning how to generate diverse background-aware instances of object shape and texture. 


%\kimki{Not sure if we need to stress this; From here:} \ag{Agreed} One advantage of this approach is that it can be trained on any dataset with mask supervision. \kimki{Till here.} 

% \ow{cite inspiration from finegan?}

% \ow{discuss how our method is evaluated}
%We train our algorithm on four classes from the diverse COCO dataset~\cite{a}, and demonstrate qualitatively that our algorithm is indeed able to capture the shape manifold of each class, and subsequently generates realistic textures in accordance with existing backgrounds collected outside from COCO dataset. 

% In summary, our algorithm presents the following contributions:
% \begin{enumerate}
%     \item It is able to generates a localized object given a user-provided bounding box.
%     \item It is able to generate multiple shapes given the same bounding box coordinates.
%     \item It is able to generate multiple textures given the same generated shape.
% \end{enumerate}



==> src/2-relatedwork.tex <==

\section{Related Work}

\vspace{-0.15cm}
\paragraph{Image compositing:} Compositing has a long history of use in graphics and vision research~\cite{perez2003poisson,agarwala2004interactive}.
Recently, we have seen that applying deep neural networks to the problem has created a set of powerful new applications. 
Deep Image Harmonization~\cite{tsaiCVPR2017} trains a neural network to realistically change the lighting and fine texture of a given foreground region by considering context from segmentation maps. 
STN-GAN~\cite{lin2018st} takes a background image and foreground object, and performs a low-dimensional warp on the foreground object to make its appearance more natural.
Similarly, SEI-GAN~\cite{ostyakov2018seigan} learns to insert an existing object into another image. 
While our goal is related, we learn how to generate \emph{new} instances of the object class rather than amend an existing image. 
We do this by generating a space of realistic foreground shapes such that the object is geometrically consistent with the observed background, and then full in the corresponding texture such that the foreground is correctly blended with the background.

%SHOULD WE CITE MORE? OR A REVIEW PAPER AT LEAST?
\vspace{-0.25cm}
\paragraph{Generative Adversarial Networks (GANs):} 
GANs have shown tremendous progress in learning-based image generation~\cite{goodfellow2014generative}. 
Networks like StyleGAN~\cite{karras2018style} can produce realistic results; however, they generate entire images, and have been shown to perform best on datasets with restricted variability (e.g., aligned faces or street scenes). 
In particular, background variability can causes GAN generators to produce blurry outputs.
This is a problem in the case of image classes with large background variability, like the animal classes in COCO, and often leads to a significant decrease in quality. 
Gau-GAN~\cite{park2019SPADE} uses semantic segmentation to provide hints about the shape and location of each object in the scene. 
%These segmentations are fed into the generative models using spatial adaptive normalization. 
However, since their technique generates images only from a segmentation map, it cannot be easily applied to existing background images. 
Zhan et al.~\cite{zhan2019adaptive} demonstrate image composition by learning geometric transforms on existing instances, but this technique does not generate new object shapes and textures. 
Unpaired image translation networks~\cite{kim2017learning,multimodal2018,zhu2017unpaired, mejjati2018unsupervised} perform fully automated domain translation, but struggle to cope with larg deformations~\cite{Gokaslan2018} making them unsuitable for object stamping. 
Instead, our goal is to generate a realistic foreground object which integrates into an existing background image, which cannot be easily accomplished with these methods.
%We condition the mask shape generator with spatial information via the object bounding box.
%Then, we combine the output shape with a texture generation network which we condition upon the existing background content. 
%Thus, our training is entirely focused on the foreground; it is not distracted by the background generation. In fact, the role of the background in our algorithm is solely devoted to transfer illumination and perspective to our generated foreground.



%https://www.cc.gatech.edu/~alanwags/DLAI2016/16.%20(Kwak+)%20Generating%20Images%20Part%20by%20Part%20with%20Composite%20Generative%20Adversarial%20Networks.pdf

%This can limit the potential usability of these algorithms as 1) They need to train on clean data, 2) the produced foregrounds need to be scaled back to the desired scale which can destroy the aspect ratio and hence the realism of the generated foreground, 3) since the training images have been centered and scaled before hand, the input image contains only little information about the background, which makes generating a foreground with realistic illumination and contrast, challenging.  

%\ow{maybe instead of these complaints, we can highlight more of our contributions. something like: In our work, we take advantage of these approaches, and train a simplified foreground generator (with isolated, aligned instances), but combine the output with an inpainting network that can be conditioned on existing background content.... } \ym{ps: we do not build upon these approaches + our input or not aligned and centered, but I have added some of  our contributions in the last paragraph}


\vspace{-0.25cm}
\paragraph{Curriculum image generation:}
Singh \etal's FineGAN~\cite{finegan} can generate convincing images from a database of a given class by separating the operation into sequential background and foreground generation. 
Composite-GAN~\cite{kwak2016generating} and LRGAN~\cite{yang2017lr} similarly recursively generates the background and foreground, but do not disentangle shape and appearance in the same way as FineGAN.
These approaches demonstrate the power of decomposed generation, and our method is inspired by such an approach. 
Our work differs in a number of ways.
For one, we generates a foreground with respect to an \emph{existing} background. 
Furthermore, our method allows for control over the location and scale of the generated foreground object conditioned on the background content. 
%Singh et al.'s problem does not have these freedoms and so their method generates centered subjects. 

Most similar to our work, Hong \etal~\cite{HierarchicalSemanticImageManpulation} `complete' a user bounding box by generating an object instance.
Our model has several differences: we can generate multiple object shapes and textures, we use the entire background for conditioning, which improves harmonization, and we generate content for the mask region only, which improves result quality. 
We compare our result directly with this approach, and show that we can generate results with overall higher quality and instance diversity.
%In sum, our approach can produce higher-quality results at lower cost and with more flexibility.


%\kimki{We are not aware of any existing algorithms tailored for object composition scenarios that we address. Here, we discuss existing algorithms in related problem domains where our algorithm design choices have been inspired from.}

==> src/3-method.tex <==
\section{Method}
\label{sec:Method}

\vspace{-0.15cm}
Our model takes as input a background image $i\in \mathbb{R}^{W\times H\times 3}$ of width $W$ and height $H$ drawn from a domain $\mathcal{I}$, a bounding box $\mathbf{b}\in\mathbb{R}^4$ containing rectangle vertices, and an object class $c$.
%in image-relative coordinates: $\mathbf{b}= [x_1/W, y_1/H, x_2/W, y_2/H]$, 
From $\mathbf{b}$, we construct a binary bounding box \emph{mask image} $b\in \mathbb{R}^{W\times H}$ with the region inside the box set to 1, and 0 otherwise.

The goal is to generate an object stamp inside the bounding box and to composite it with the background image $i$ (Figure~\ref{fig:architecture}).
%The stamp $\hat{s}$ should be seamlessly incorporated into $i$ such that $i_{\hat{s}}$ cannot be discriminated from the images in $\mathcal{I}$.
We achieve this by first generating a stamp mask $\hat{m}\in\mathbb{R}^{W\times H}$, and then generating a textured stamp $\hat{s}\in\mathbb{R}^{H\times W\times3}$ such that when composited into the final image $i_{\hat{s}}=i\odot(1- \hat{m}) + \hat{s}\odot\hat{m}$, $i_{\hat{s}}$ is indistinguishable from images in $\mathcal{I}$.

% \zs{During training, the input image $i$ is taken from the COCO dataset and so contains object instances. Therefore, we can have the ground truth stamp shape mask $m$, texture $s=i\odot m$, and $i_s =i$ . However, during inference, there is no such object in the bounding box (Figure~\ref{fig:architecture}).}
%As training a network to generate such stamps is ill-posed, we stratify training across two stages: 1) stamp shape mask generation and 2) stamp texture generation. Each stage is a conditional generation problem, which we train adversarially 




%\kimki{I guess $\mathcal{I}$ represents a finite sample (\ie training set) not the domain of images when we say ``discriminated from the images in $\mathcal{I}$''? Later, we use `$\mathbb{R}^{W\times H\times 3}$' to denote the image domain. Then, can we clearly state that ``Given an input image $i$ ..... cannot be discriminated from the sample images $\mathcal{I}$''?} 


% \kimki{Do we need hat ($\hat{s}$) for $s$?}\zs{Since the stamp is generated by our model, I'd like to use hat to differentiate from the ground truth.}

%\zs{We begin with an overview of the proposed pipeline in \ref{sec:Method-overview}, and we will go through the details of each component in the subsequent subsections.}

%% \zs_comment Our method consists of two steps: learning to synthesize object shapes from a database of binary masks $\M$, and learning to synthesize object texture from a corresponding database of images $\I$ (Fig.~\ref{fig:architecture}). Architecture details for all networks are provided in the supplementary material.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \zs_comment\subsection{Learning to synthesize object\zs{stamp} shapes} 


%%%%%%%%%%%%
% Variables & naming
%
% \I = database of images
% \M = database of masks
% i = an image
% m = a mask

% D = discriminator
% G = generator
% G_I, G_M, D_I, D_M = image/mask generators/discriminators

% b = bounding box
% \z_m = random latent vector used per sample (is that right? is z per sample?)
% |\z_m| = number of entries in z_m; saves introducing n

% \Theta = network parameters
%\paragraph{Image input and preprocessing.} 
%% , we select the models $G_M$ and $G_T$ trained on class $c$ for further processing.



%\vspace{-0.25cm}
%\paragraph{Final results:} Given the stamp $\hat{s}$, the model generates the final image: $i_{\hat{s}}=i\odot(1- \hat{m}) + \hat{s}\odot\hat{m}$. For the user, an input image and bounding box can generate diverse outputs from $G_M$ and $G_T$ via $\mathbf{z}_m$ and $\mathbf{z}_t$, both of which can vary via the background content.

%% \zs_comment
% We wish to train a network $G_M$ to generate an object mask (real valued; $[0,1]$) which fools a discriminator $D_M$. Given a training database image $i \in \I$ containing at least one instance of a given class, \kimki{CVPR recommends \eg over `e.g.':} e.g., `giraffe', we randomly pick an instance. Given its binary mask $m \in \M$, we create a vector $b$ which describes the bounding box location of the object: if $[x_1, y_1]$ and $[x_2, y_2]$ are the top left and bottom right coordinates, and $h$ and $w$ are the height and width of the image, then $b = [\frac{x_1}{h}, \frac{y_1}{w}, \frac{x_2}{h}, \frac{y_2}{w}]$. 
% Next, we form the background conditioning image $i_c$ by setting the region within the bounding box (containing the giraffe) to black. 
% Further, to learn to generate diverse examples via stochasticity, we condition mask generation on a randomly sampled latent variable $\z_m$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \includegraphics[clip,width=0.8\linewidth]{figures_cvpr/Shape.pdf}
    % \includegraphics[clip,width=0.495\linewidth]{figures_cvpr/Texture.pdf}
    \caption{\emph{Our stamp shape generation model.} This generates a shape mask $\hat{m}$ given a random vector $\mathbf{z}_m$ and input image $i_b$ with bounding box region zeroed-out. We use a discriminator $D_M$ and adversarial loss $\mathcal{L}_{\text{Adv}}^M$ to train the generator. We apply a feature matching loss $\mathcal{L}_{\text{FM}}^M$ on $\hat{m}$ to improve the generation quality. AdaIN injection of $\mathbf{z}_m$ and $\mathbf{b}$ improves the generator. Finally, we add a random vector reconstruction loss $\mathcal{L}_{\text{Rec}}^M$ to maintain the diversity of generated shapes.}
    \label{fig:architecture-shape}
    \vspace{-0.25cm}
\end{figure}

\subsection{Stamp shape generation model}
\label{sec:Method-shape}

We train a generator $G_M$ conditioned on a random vector $\mathbf{z}_m$ drawn from a Gaussian with mean 0 and variance 1: $\mathbf{z}_m \sim \mathcal{N}(0,I)$, as well as the bounding box and background image.
Importantly, we train the generator on images that contain object instances and their respective masks.
Therefore, to allow us to condition on background content at test time that does \emph{not} contain the object in question, we first zero-out the bounding box region $i_b=i\odot(1- b)$, $\odot$ is the element-wise product.
This prevents the network from trivially learning to segment existing instances in the training data.
% of $i$ (during training, $b$ already contains object instances \ow{is this right?})

The generator $G_M$ produces a binary mask $\hat{m}$ for the shape of the stamp object inside the bounding box region, \eg  $\hat{m} = G_M(i_b, \mathbf{z}_m)$. 
%Since the input $i_{b}$ contains only the texture outside the box region, $G_M$ will learn to generate the unseen shape conditional on the given background. 
We train $G_M$ adversarially: $G_M$ attempts to generate realistic shapes to fool a discriminator $D_M$, while $D_M$ attempts to classify generated masks separately from real training data masks. 
$D_M$ is a CNN which takes as input the shape mask and corresponding bounding box: $D_M(m,b)$ 
We use a hinge-GAN loss $\mathcal{L}^M_{\text{Adv}}$ to train both $G_M$ and $D_M$ for better stability~\cite{lim2017geometric,tran2017deep,miyato2018spectral}:
%
% $G_M$ attempts to generate realistic shapes to fool $D_M$, while $D_M$ attempts to classify generated masks from training data masks.
%
% \zs{I did not mention the tile part (``we tile the vector $b$ into a $w\times h \times 4$ array and concatenate it with $m$'') here, because that does not sound intuitive for me. So what's your point here? Should we mention that or not?}
%
\begin{align}
    \mathcal{L}^M_{\text{Adv}}(G_M,D_M) = & \mathbb{E}_{m}{[\min(0, D_M(m,b)-1)]} + \nonumber \\ 
    &\mathbb{E}_{\hat{m}}{[ \min(0,-D_M(\hat{m},b))-1]},
    \label{eq:Loss_M_Adv}
\end{align}
where $m$ is a ground-truth shape mask and $\hat{m}$ is generated. 
% \zs{I just shifted the signs here, following some other examples in \url{https://arxiv.org/pdf/1901.08753.pdf} (Table 1). What's your opinion? (also here \url{https://arxiv.org/pdf/1808.07535.pdf})}
%% Old one:
% \begin{align}
%     \calL_{D_M}&(\Theta_{D_M}) = \\
%               &-\E_{\z_m \sim \mathcal{N}(0,\,I)}(\min(0, -D_M(m', b)-1)) \nonumber \\
%               &-\E_{m\in \M}(\min(0, D_M(m,b)-1)), \nonumber \\
%     \calL_{G_M}&(\Theta_{G_M}) = -\E_{\z_m \sim \mathcal{N}(0,\,I)}(D_M(m', b)),
% \label{eq:hingeLSGANmask}
% \end{align}
% 
% 
%

%We use AdaIn to preserve the shape dependence on the random vectors, and perceptual and feature matching losses to improve generation quality (Sec.~\ref{sec:Method-shape}).
Next, we describe how we use adaptive instance normalization (AdaIN)~\cite{huang2017adain} in $G_M$ to condition the network on the input noise $\mathbf{z}_m$.
%This method has seen success in style transfer~\cite{huang2017adain, multimodal2018,karras2018style,romero2018smit} to inject auxiliary information into the output of convolutional layers. 
In our case, we wish to inject the bounding box $b$ and the latent vector $\mathbf{z}_m$ during shape generation. 
For this, similar to prior work~\cite{huang2017adain}, we use a small fully-connected feed-forward network (MLP) encoder $\text{Enc}^M$ to take input $b$ and $\mathbf{z}_m$ and predict affine transformation parameters $\text{Enc}^M(b,\mathbf{z}_m)$ for the instance normalization layers.

One issue we found is that AdaIN can learn to ignore $\mathbf{z}_m$ by using only $b$, which reduces diversity in generation. 
To overcome this, we apply a novel reconstruction loss $\mathcal{L}^M_{\text{Rec}}$ over $\mathbf{z}_m$ via an MLP decoder complement $\text{Dec}^M$ to $\text{Enc}^M$:
\begin{align}
    \mathcal{L}^M_{\text{Rec}}(\text{Enc}^M, \text{Dec}^M) = \frac{1}{|\mathbf{z}_m|}{\|\mathbf{z}_m - \text{Dec}^M(\text{Enc}^M(b, \mathbf{z}_m))\|_1^2}.
    \label{eq:Loss_M_Rec}
\end{align}
% \zs{where $|\mathbf{z}_m|$ is the $L_2$ norm of vector $\mathbf{z}_m$, and $||\cdot||_1$ is the $L_1$ norm.}  % \JT{We don't need to spell this out.}
Unlike prior work~\cite{zhu2017bicycle}, $\text{Dec}^M$ decodes the latent vector from $\text{Enc}^M(b,\mathbf{z}_m)$ rather than the output mask $\hat{m}$, which we found to perform better in our experiments.
This loss directly enforces that the AdaIN parameters depend on the random vector $\mathbf{z}_m$, and so helps to maintain diversity.

This yields diverse results, but we found that the masks lacked fine detail.
Therefore, we propose a variant on the commonly used deep feature matching loss~\cite{salimans2016improved,zhang2018unreasonable}, which has been shown to enhance image sharpness by enforcing that real and generated images elicit similar feature responses in each layer $l$ of the discriminator $D_M^{(l)}$, via a squared $L_2$ norm.
In our case, since our generated mask $\hat{m}$ does not match a single real mask, but rather a \emph{distribution} (\eg it varies by $\mathbf{z}_m$), we cannot directly compare the feature responses from ground truth masks $m$ with $\hat{m}$.
Instead, we compute a moving average of the feature response from each batch of training examples $\bar{D}_M^{(l)}$ to obtain a \emph{mean distribution} of the training shapes for comparison:
\begin{align}
    \mathcal{L}^M_{\text{FM}}(D_M) = \mathbb{E}_{\hat{m}, m}\sum_{l=1}^{L}||{D_M^{(l)}(\hat{m},b) - \bar{D}_M^{(l)}(m,b)}||_2^2.
    \label{eq:Loss_M_FM}
\end{align}
This approach is the first we know of to show that such a minibatch feature matching loss can be used to generate sharp \emph{binary} image masks.
%where $D_M^{(l)}$ is the output of the $i$-th layer in $D_M$, and $||\cdot||_2$ is the $L_2$ norm. 
%
%\zs{We apply a modified feature matching loss, where the comparison target $\bar{D}_M^{(i)}(m,\mathbf{b})$ is the moving average of layer $i$'s output across different samples in the training set. Since our generated mask $\hat{m}$ is variable to $\mathbf{z}_m$, we cannot directly match ground truth masks $m$ with $\hat{m}$. Instead, we use the feature response $\bar{D}_M^{(i)}(m,\mathbf{b})$ averaged from multiple training samples to obtain the \emph{mean distribution} of the training shapes for comparison. }

% \kimki{A note for future work, we could use distribution matching \eg MMD here.}

Our combined learning objective for the stamp shape mask generator $\mathcal{L}^M$ is a weighted combination the aforementioned losses:
\begin{align}
    \mathcal{L}^M = \mathcal{L}^M_{\text{Adv}}+ \lambda^M_{\text{FM}}\mathcal{L}^M_{\text{FM}} + \lambda^M_{\text{Rec}}\mathcal{L}^M_{\text{Rec}},
    \label{eq:Loss_M}
\end{align}
where $\lambda^M_{\text{FM}}$, $\lambda^M_{\text{Rec}}\geq 0$ are hyperparameters.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We pass $i_c$ as input to $G_M$, and we inject $b$ and $\z_m$ into $G_M$ via adaptive instance normalization (AdaIN)~\cite{huang2017adain}.
% Specifically, we concatenate $b$ and $\z_m$ into a conditioning vector, then we pass this through a Multi-Layer Perceptron (MLP) which predicts the parameters of an affine transformation applied to the Instance Normalization layers. 
% This approach has seen success in style transfer applications~\cite{huang2017adain, multimodal2018,karras2018style,romero2018smit}. 
% However, $b$ and $\z_m$ could be ignored: na\"{i}ve injection does not ensure that the generated mask will be wholly contained within the user-defined bounding box, nor that the mapping will be stochastic.

% To preserve the bounding box constraints, we condition our mask discriminator network $D_M$ on $b$: we tile the vector $b$ into a $w\times h \times 4$ array and concatenate it with $m$.
% This ensures that the generated masks are realistic, and that they agree with $b$ in the same way that real masks agree with $b$.

% To preserve mask stochasticity, we use a reconstruction loss on $\z_m$:
% % \kimki{(with $|\z_m|$ being the dimensionality of $\z_m$)}:
% \begin{align}
%     \calL^M_{rec}(\Theta_{G_{M}}) = \frac{1}{|\z_m|} \left\| \z_m - \text{Enc}_m( \text{MLP}(\z_m, b))\right \|_1^2,
%     \label{eq:maskzrecloss}
% \end{align}
% where $\Theta_{G_{M}}$ are the learnable parameters of $G_M$, $\text{MLP}$ predicts the affine parameters of the AdaIN layers, and $\text{Enc}_m$ is a fully-connected encoder trained to reconstruct $\z_m$. 
% In contrast to other algorithms~\cite{multimodal2018,zhu2017bicycle}, we do not reconstruct $\z_m$ from the image but rather \emph{directly} from $\text{MLP}(\z_m,b)$ as we find it to give better results.
% It is not easy for the network to ignore variance in AdaIN parameters, and this approach essentially forces the AdaIN parameters to vary with respect to $\z_m$.


% We train $D_M$ and $G_M$ using the hinge-GAN loss, which is known for its training stability \cite{lim2017geometric,tran2017deep,miyato2018spectral}:\kimki{Can we use $\mathbb{E}$ instead of $\mathcal{E}$ to denote an expectation?}
% \begin{align}
%     \calL_{D_M}&(\Theta_{D_M}) = \\
%               &-\E_{\z_m \sim \mathcal{N}(0,\,I)}(\min(0, -D_M(m', b)-1)) \nonumber \\
%               &-\E_{m\in \M}(\min(0, D_M(m,b)-1)), \nonumber \\
%     \calL_{G_M}&(\Theta_{G_M}) = -\E_{\z_m \sim \mathcal{N}(0,\,I)}(D_M(m', b)),
% \label{eq:hingeLSGANmask}
% \end{align}
% where $m'=G_M(i_c, \z_m, b)$ is the generated mask (real values in $[0,1]$), and $\Theta$ is the respective set of network parameters. \kimki{``and $\mathcal{N}(0,I)$ denotes the standard normal distribution.''} \kimki{What don't we use $\mathcal{N}$ (instead of $\mathcal{N}(0,1)$) and define it as the standard normal distribution?}

% Furthermore, we enhanced the perceived quality of the reconstructed image by adopting the deep feature matching loss~\cite{salimans2016improved,zhang2018unreasonable}.
% Such a loss enforces that the real and generated images produce similar feature responses in terms of the squared $L_2$ norm on each layer of the discriminator: 
% \begin{align}
%     \calL^M_\text{\emph{FM}}(\Theta_{G_M}) = \sum_{l=1}^{L_{D_M}} \E_{\z_m \sim \mathcal{N}(0,\,I)}( \left\|D_M^l(m', b)- \bar{d}^l_m \right\|_2^2),
%     \label{eq:maskFM_loss} 
% \end{align}
% where $L_{D_M}$ is the number of layers in $D_M$ and $\bar{d}^l_m$ is the moving average at layer $l$ of $D_M^l(m,b)$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    %\includegraphics[clip,width=0.495\linewidth]{figures_cvpr/Shape.pdf}
    \includegraphics[clip,width=0.8\linewidth]{figures_cvpr/Texture.pdf}
    \caption{\emph{Our stamp texture generation model.} We train a generator $G_T$ via a discriminator $D_T$. Feature match $\mathcal{L}^T_{FM}$, perceptual $\mathcal{L}^T_{Per}$, and auxiliary losses $\mathcal{L}^T_{Rec}$ help to simultaneously maintain fine texture detail and diversity, while conditioning on random vector $\mathbf{z}_t$ provides user control.}
    \label{fig:architecture-texture}
    \vspace{-0.25cm}
\end{figure}
\subsection{Stamp texture generation model}
\label{sec:Method-texture}

The goal of the texture generator $G_T$ is to create realistic textures that match the pose contained in the shape mask (e.g., frontal \vs profile) and the lighting and shading to match the background. 
%Depending on the application, the shape mask could be either 1) $\hat{m}$ predicted from a given bounding box, or 2) $m$ provided directly by the the user.
%For simplicity, we refer to the shape mask as $m$ during this section.
Given a generated shape mask $\hat{m}$, we first cut out (set to zero) the shape from the input image to mark the area that needs texturing: $i_{\hat{m}}=i\odot(1-\hat{m})$. 
Then, the stamp texture generation $G_T$ synthesizes the texture inside the empty region while still having access to the texture of the surrounding background: $\hat{s}=G_T(i_{\hat{m}}, \mathbf{z}_t)$. 
$\hat{s}\in\mathbb{R}^{H\times W\times3}$ is the generated object stamp image, and $\mathbf{z}_t \sim \mathcal{N}(0,I)$ is a random vector to add stochasticity for diverse generation. 
For $G_T$, we use a BicycleGAN-like \cite{zhu2017toward} architecture to preserve both texture quality and diversity.
Similar to $G_M$, $G_T$ is trained adversarially via a texture discriminator $D_T$.
%Our stamp texture generator $G_T$ is conditioned on a given shape mask and background image. 
%Depending on the application, the shape mask could be either 1) $\hat{m}$ predicted from a given bounding box, or 2) $m$ provided directly by the the user.
%For simplicity, we refer to the shape mask as $m$ during this section.
%it takes as input the final image composite $i_{\hat{s}}$ and the shape mask $m$, which allows it to judge how well the predicted stamp texture matches the background.

%\paragraph{Diversifying texture generation:} 
%Our approach is related to that for the mask; however, 
%and so cause object details not to be captured, which is less of a problem for \emph{binary} masks which, by their construction, must contain sharp edge details. 
%As such, we need a new way to combine randomly-generated textures against ground-truth textures.

% \JT{1) possible: Argument is that easier to train a mask generator, and so moving average is sufficient. 2) possible: diversity in mask data is higher, more erroneous, so moving average is needed.}
% \JT{Did Youssef try the mask generator with the BicycleGAN trick?}
% \kimki{Another possible 3) We observed in our preliminary experiments that for binary masks, comparing two distributions based on their moving averages does not blur individually generated masks. This is not the case for RGB textures.} \ym{I tried bicycle gan on masks using a reduced dataset, and it collapses. Did not have time to proerly inverstigate why this was the case.}\kimki{OK. So it means that indeed, applying this strategy is non-trivial... }

The input to the discriminator $D_{T}$ is the channel-wise concatenation of the real tuple $(i_s,m)$ or the fake image tuple $(i_{\hat{s}},\hat{m})$. 
Passing the mask to $D_T$ essentially tells the discriminator to expect an instance of the object at that location. 
This is important, as at training time, the background image $i_{\hat{s}}$ may contain \emph{multiple} instances of the target class, and so $D_T$ would be satisfied by the generator simply filling in the background.

Unlike $D_M$, we do not use a moving average feature matching loss as we found it to blur the feature responses and cause the generator to miss object details.
Instead, we use a CNN to encode the ground-truth texture of $s=i \odot m$ as a latent vector $\mathbf{z}_t'=\text{Enc}^T(s)$, and then use $\mathbf{z}_t'$ and $m$ to generate another stamp texture $\hat{s}'=G_T(i_m,\mathbf{z}_t')$ and corresponding stamped image $i_{\hat{s}'}=i\odot(1-m)+\hat{s}'\odot m$. 
As $\mathbf{z}_t'$ depends on $s$, this indirectly conditions $i_{\hat{s}'}$ on $s$, and allows us to apply a feature matching loss without losing detail:
\begin{align}
    \mathcal{L}^T_{\text{FM}}(D_T) = \mathbb{E}_{i_{\hat{s}'}, i_s}\sum_{l}||{D_T^{(l)}(i_{\hat{s}'},m) - D_T^{(l)}(i_s,m)}||_1^2.
    \label{eq:Loss_T_FM}
\end{align}
Here, $D_T^{(l)}$ is the output of the $l$-th layer in $D_T$. 
An additional $L_1$ image reconstruction loss $\mathcal{L}^T_{\text{iRec}}$ were also applied to facilitate the texture filling: $\mathcal{L}^T_{\text{iRec}} =\frac{1}{|i_s|}\sum_{l=1}||{i_{\hat{s}'}- i_s}||_1^2$.
%Further helping the texture filling is a reconstruction loss on the image itself: 

% \begin{align}
%     \mathcal{L}^T_{\text{iRec}} = \frac{1}{|i_s|}\sum_{l=1}||{i_{\hat{s}'}- i_s}||_1^2.
%     \label{eq:Loss_T_iRec}
% \end{align}
% \ym{until here}

% We use a squared $L_1$ norm to generate sharp edges. 
% \JT{Masks also need sharp edges! Why don't we do that for masks? A bit odd...} 
% \ym{For the masks we use a feature moving average on the FM loss rather than pairwise differences: We want feature activations to be similar on average, which is better represented by the L2 loss}
% \kimki{I think James' question is about why we want them similar on average...} 
% \ym{Because for the masks we don't have ground truth data, as the masks generated are completely random.}
%

As an extra constraint on $\mathbf{z}_t'$, we wish for its distribution $\mathcal{Z}_t'$ to be similar to the distribution of $\mathbf{z}_t$, such that the generator $G_T$ cannot use any distribution difference to fool $D_T$. 
Thus, we use the re-parametrization trick~\cite{kingma2013auto} on $\text{Enc}$, and add a KL-divergence loss $\text{KL}(\mathcal{Z}_t'||\mathcal{N}(0,I))$ to promote distribution consistency. 
%\JT{This content is not yet integrated; it may be important...:
%``We facilitate the sampling at test time and we avoid large values in $z'_i$ by enforcing it to be sampled from a random normal distribution. 
%We achieve this by using the re-parametrization trick~\cite{kingma2013auto} on $\text{Enc}$, then we add a KL loss between $z'_i$ and a randomly sampled vector $q\sim \mathcal{N}(0,\,I)$ of the same shape.''}

%Given this positive outcome, one might consider applying the same BicycleGAN-like~\cite{zhu2017toward} approach to masks instead of the moving average technique. However, preliminary experiments with this auxiliary latent encoding on masks led to mode collapse. %, \JT{posit an explanation? or just say `and further investigation is required'.}

\vspace{-0.25cm}
\paragraph{Texture architecture:}
Compared to our mask architecture, we make five changes for our texture model. First, unlike for masks, for texture there is no need for an AdaIN component to inject auxiliary information into the generator: Since $D_T$ is trained on the full image $i_s$ and $i_{\hat{s}}$, the generator must use the shape information even without AdaIN. 

Second, we penalize a latent vector texture reconstruction loss on $\mathbf{z}_t$ via an encoder on $\hat{s}$:
\begin{align}
    \mathcal{L}^T_{\text{Rec}}(\text{Enc}^T) = \frac{1}{|\mathbf{z}_t|}{||\mathbf{z}_t - \text{Enc}^T(\hat{s})) ||_1^2}.
    \label{eq:Loss_T_Rec}
\end{align}

Similar to~\cite{zhu2017toward}, we do not update $\text{Enc}^T$ when propagating the gradients from Eq.~\ref{eq:Loss_T_Rec}. This avoids that $\text{Enc}^T$ hides information in the data, making it easy to reconstruct~\cite{chu2017cyclesteg}.

Third, we use both $i_{\hat{s}}$ and $i_{\hat{s}'}$ to train $G_T$ and $G_M$, and so the adversarial loss $\mathcal{L}_{\text{Adv}}^T$ becomes:
\begin{align}
    \mathcal{L}^T_{\text{Adv}}(G_T,D_T) = \
    &\mathbb{E}_{i_s}{[\min(0, D_T(i_s,m)-1)]} + \nonumber \\
    &\mathbb{E}_{i_{\hat{s}}}{[\min(0, -D_T(i_{\hat{s}},m)-1)]} + \nonumber \\ 
    &\mathbb{E}_{i_{\hat{s}'}}{[\min(0, -D_T(i_{\hat{s}'},m)-1)]}.
    \label{eq:Loss_T_Adv}
\end{align}

Fourth, we add a perceptual loss~\cite{johnson2016perceptual} to help recreate fine textural details, \eg, the tail of a giraffe.
This loss uses a pre-trained VGG16 network to extract features for two image instances, then enforces that their feature activations are as similar as possible:%. We use the features from the third hidden layer from the input:
%, i, i_{\hat{s}}
\begin{align}
    \mathcal{L}^T_{\text{Per}}(G_T) = \frac{1}{N} \left\|\phi(i) - \phi(i_{\hat{s}'})\right\|_1^2,
    \label{eq:Loss_T_Per}
\end{align}
where $\phi(i)$ is the third layer output the VGG16 network, and extracts $N$ features from $i$.

Fifth, and finally, we add Gaussian noise $\mathcal{N}(0,I)$ to the texture decoder \emph{a la} StyleGAN~\cite{karras2018style}. This helps the diversity of the results and improves image generation quality (Table~\ref{tab:KIDtexture}).

The overall texture generation training loss $\mathcal{L}^T$ is:
\begin{align}
    \mathcal{L}^T =  
    \mathcal{L}^T_{\text{Adv}} 
  &+\lambda^T_{\text{Rec}}\mathcal{L}^T_{\text{Rec}} +
     \lambda^T_{\text{KL}}\text{KL}(\mathcal{Z}_t'||\mathcal{N}(0,I))  \nonumber \\ 
  &+\lambda^T_{\text{FM}}\mathcal{L}^T_{\text{FM}} +
     \lambda^T_{\text{Per}}\mathcal{L}^T_{\text{Per}} + 
     \lambda^T_{\text{iRec}}\mathcal{L}^T_{\text{iRec}},
    \label{eq:Loss_T}
\end{align}
where $\lambda^T_{\text{Rec}}$, $\lambda^T_{\text{KL}}$, $\lambda^T_{\text{FM}}$,$\lambda^T_{\text{Per}}$,and $\lambda^T_{\text{iRec}}\geq 0$ are hyperparameters. 
$\lambda^T_{\text{Rec}}$ and the $\text{KL}$ divergence increase diversity, while the $\lambda^T_{\text{FM}}$, $\lambda^T_{\text{Per}}$, and $\lambda^T_{\text{iRec}}$  improve the quality of the generated texture.
We present a detailed architecture description in the supplemental material.

% \zs{The stamp texture is generated conditional on the given shape mask and surrounding image backgrounds. Good texture should provide the shape with distinguished visual properties and reflects the varied lighting, shadows, etc., in the background. Since the object texture lies in color image manifold, it has larger variability than binary shape masks. Therefore, besides the current methods used in training $G_m$ and $D_m$, extra design need to be applied to facilitate the training of the generator $G_T$ and 


% \paragraph{Instance-aware discrimination:}
% The inputs to the discriminator $D_{M}$ are the channel-wise concatenation of the real tuple $(i,m)$ and the fake image tuple $(i_{\hat{s}},\hat{m})$. 
% It might seem like $D_{M}$ should only need to see $i$ \emph{or} $i_{\hat{s}}$ to tell whether an object has been realistically textured against a background. 
% However, without $m$, our generator will eventually learn to texture the object mask \emph{with background} because some database images contain multiple object instances: Suppose there are two giraffes in an image, and our generator must learn to texture the first giraffe mask. The generator could place background-like texture, which is easier, and $D_{M}$ would \emph{still be satisfied} that the image is real by its observation of the second giraffe instance. Explicitly forcing $D_{M}$ to observe only giraffe regions forces the generator to texture as desired.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Forward declaration of results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\import{\figDirCVPR}{fig_zebra}
%\import{\figDirCVPR}{fig_giraffe}
% \import{\figDir}{fig_bus}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%\subsection{Learning to synthesize object texture}
% We can now generate realistic masks conditioned on a user's bounding box and background image. Our next goal is to texture the mask.
% To do this, we train an object texture generator $G_{I}$ using a general image adversary network $D_{I}$, which is trained as a real/fake classifier assessing the quality of both the generated texture as well as how it blends with the background.
% %Inspired by Zhu et al's bicycle GAN~\cite{zhu2017bicycle} and 
% % Both are trained as a real/fake classifiers and see real object instances, with $D_I$ seeing them against real backgrounds.
% In addition, we want to enforce stochastic texture generation to represent variation in object appearance. 

% Given a real image $i \in \I$ and a mask $m \in \M$ for a single object instance in $i$, the input to the generator $G_{I}$ is the masked real background $s = i\circ(1-m)$, where $\circ$ is the element-wise product, and a latent vector $\z_i$ to enforce stochasticity in the texture generation. 
% $\z_i$ is concatenated layer-wise into the encoding part of $G_{I}$. Similar to Eq.\ref{eq:maskzrecloss}, we encourage a stochastic texture generation process via a latent reconstruction loss $\calL^I_{rec}$ on $\z_i$:
% \begin{align}
%     \calL^z_{rec}(\Theta_{G_{I}}, \z_i) = \frac{1}{|\z_i|} \left\|\z_i - \text{Enc}(s'\circ m)\right\|_1^2.
%     \label{eq:zrec}
% \end{align}

% In Eq.~\ref{eq:zrec}, we reconstruct the latent vector from the generated foreground $s'\circ m$~\cite{zhu2017bicycle}. 
% %
% Then, we create composite image $s'$ from the element-wise sum of generated object and real background:
% \begin{align}
%     s' &= G_{I}(s, \z_i) \circ m + i \circ (1-m).
%     \label{eq:s'}
% \end{align}

% To improve the details in our generated images we impose a set of reconstruction and feature matching losses. First we use a pixel-wise reconstruction loss: 
% \begin{align}
%     %\calL^i_{rec}(\Theta_{G_{I}}, s') = \frac{1}{\left\|m\right\|_0} \left\|i - s'\right\|_1^2,
%     \calL^i_{rec}(\Theta_{G_{I}}, s') = \frac{\|i - s'\|_1^2}{\|m\|_0},
%     \label{eq:irec}
% \end{align}
% where we normalize by the sum of non zero elements in $m$ to equally account for instances of different sizes.  
% When doing so, Eqs.~\ref{eq:zrec},~\ref{eq:irec} serve contradictory purposes.
% Indeed, doing so encourages our network to reconstruct $i$ from a random latent vector $z_i$ that differs from an epoch to the other. 
 
% To account for this, we use an additional latent vector $\z'_i$, which we obtain by encoding the real foreground: $\text{Enc}(i \circ m)=\z'_i$. Then, using~\ref{eq:s'} and $\z'_i$, we generate the image $s''$ which is applied as input to Eq.~\ref{eq:irec} instead of $s'$.

% Adding a perceptual loss~\cite{johnson2016perceptual} helps recreate fine textural details, e.g., the tail of the giraffes in Fig~\ref{}.
% This loss uses a pre-trained VGG16 network to extract features for two image instances, then enforces that their feature activations are as similar as possible. We use the features from the third hidden layer: 
% \begin{align}
%     \calL^i_{p}(\Theta_{p}, i, s'') = \frac{1}{N} \left\|\phi(i) - \phi(s'')\right\|_1^2,
%     \label{eq:irec2}
% \end{align}
% where $\phi(i)$ are extracted features of $i$, and $N$ its cardinal. 

% We facilitate the sampling at test time and we avoid large values in $z'_i$ by enforcing it to be sampled from a random normal distribution. 
% We achieve this by using the re-parametrization trick~\cite{kingma2013auto} on $\text{Enc}$, then we add a KL loss between $z'_i$ and a randomly sampled vector $q\sim \mathcal{N}(0,\,I)$ of the same shape.

% \paragraph{Discussion:}
% The inputs to the discriminator $D_{I}$ are the channel-wise concatenation of the real tuple $(i,m)$, and the fake image tuple $(s',m)$. It might seem like $D_{I}$ should only need to see $i$ or $s'$ to tell whether an object has been realistically textured against a background. However, without $m$, our generator will eventually learn to texture the object mask \emph{with background} because some database images contain multiple object instances: Suppose there are two giraffes in an image, and our generator must learn to texture the first giraffe mask. The generator could place background-like texture, which is easier, and $D_{I}$ would \emph{still be satisfied} that the image is real by its observation of the second giraffe instance. Explicitly forcing $D_{I}$ to observe only giraffe regions forces the generator to texture as desired.

% For training, we adopt hinge-GAN-based losses using both $s'$ and $s''$:
% {\small
% \begin{align}
%     \calL_{D_{I}}&(\Theta_{D_{I}}) = \\
%                  &-\E_{m\in \M, i \in \I}\big(\E_{\z_i \sim \mathcal{N}(0,\,I)}(\min(0, -D_{I}(s', m)-1)) \nonumber \\ 
%                  & + \E_{\z'_i}(\min(0, -D_{I}(s'', m)-1)) \nonumber \\ 
%                  &+ \min(0, D_{I}(i,m)-1)\big), \nonumber \\
%     \calL_{G_{I}}&(\Theta_{G_{I}}) = \\
%                  &-\E_{\z \sim \mathcal{N}(0,\,I), m\in \M, i\in \I, \z'_i}(D_I(s', m) + D_I(s'', m)) \nonumber,\\
%     \label{eq:hingeLSGANgt}
% \end{align}
% }%
% \kimki{Shouldn't $\E_{m\in \M, i \in \I}$ be a summation?: $\sum_{m\in \M, i \in \I}$;} \kimki{I guess in the second summand, the expectation should be written as $\E_{\z_i \sim \mathcal{N}(0,I)}$?}\kimki{Previoulsy, we used $\mathbb{E}$ (not $\mathcal{E}$) to denote the expectation operator .}
% where $\Theta_{D_{I}}$ and $\Theta_{G_{I}}$ are network parameters of $D_{I}$ and $G_{I}$ respectively. Similar to the mask generation step (Eq.~\ref{eq:maskFM_loss}), we also use a deep feature matching loss $\calL^I_\text{\emph{FM}}$, but since we have the ground truth image $i$, we do not use feature moving averages:
% {\small
% \begin{align}
%     %\calL^I_\text{\emph{FM}}&(\Theta_{G_{I}}) = \\
%      %&\sum_{l=1}^{L_{D_I}} \E_{\z'_i, m\in \M, i\in \I}\left( \left\|D_{I}^l(s'', m)- D_{I}^l(i, m) \right\|_1^2\right). \nonumber\\
%      \calL^I_\text{\emph{FM}}&(\Theta_{G_{I}}) = \\
%      &\sum_{l=1}^{L_{D_I}} \E_{\z'_i, m\in \M, i\in \I}\left(\|D_{I}^l(s'', m)- D_{I}^l(i, m) \|_1^2\right). \nonumber\\
%     \label{eq:FM_loss} 
% \end{align}
%}%
%
%
%
% 
% 
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Simultaneous generator training} 
% To allow us to train both the object mask $G_{M}$ and texture $G_{I}$ generators together, we construct $s$, the input to $G_I$, using the generated mask $m'$: $s = i\circ(1-m')$. This approach creates a gradient flow between $G_{M}$ and $G_{I}$ during training, i.e., as mask realism increases it has a potentially positive effect on texture realism. This also helps ensure that the synthesized masks $m'$ at testing do not significantly deviate from the training masks $m$.

%Again, we encourage the adversarial and feature matching losses alone in that stage does not encourage a stochastic texture generation. Indeed, if the generator ignores $z^*$ then it is still possible to minimize Eqs~\ref{eq:hingeLSGANgt},~\ref{eq:FM_loss*}. To avoid this situation we add a latent reconstruction loss on $z^*$, which enforces that the information carried in it does not get ignored:

% where $\text{MLP}$ is the Multi-Layer Perceptron used to predict the affine parameters of ADAIN layers and $\text{Enc}$ is a fully connected encoder whose job is to reconstruct $z^*$, and $n_{z^*}$ is the number of elements in $z^*$ which is set 20. Note that in contrast with other existing algorithms, we do not reconstruct $z^*$ from the image but rather directly from $\text{MLP}(z^*)$ as we find it to empirically give better results.  

% We obtain the image to be fed to the discriminator $D_I$ as:
% \begin{align}
%     %s'' = G_I(s, \z_i^*)\circ m' + i\circ (1-\b),
%     s'' = G_I(s, \z_i)\circ m' + i\circ (1-\b),
%     \label{eq:s''}
% \end{align}
% where $\b$ is a 2D binary mask where pixels inside the coordinates of $b$ are 1 and outside are 0. 

% Eq.~\ref{eq:s''} is different from the equivalent operation on real inputs, as defined in Eq.~\ref{eq:s'}. In Eq.~\ref{eq:s'}, we use all of the real background outside the mask, while in Eq.~\ref{eq:s''} we only use the background given by $i\circ(1-\b)$. This is because at training time $b$ \emph{already contains} an instance, and so replacing the background by $i\circ(1-m')$ as in Eq.~\ref{eq:s'} might `overlay' or `merge' two instances inside $b$: the generated one and the original one. This unexpected signal distorts object appearance and disturbs training. Note that Eq.~\ref{eq:s''} is only applied at training time; at test time we use Eq.~\ref{eq:s'}.  

%\paragraph{Object discriminator:}
% \noindent\textbf{Object discriminator:}
% $s'$ and $s''$ have different content: $s'$ has complete background and object texture inside $b$, but $s''$ has no background texture inside $b$. Thus, we cannot use the same adversary $D_{I}$ to train the generator $G_I$ with respect to $s''$. Instead we introduce a new object discriminator $D_{O}$ which acts as a real/fake classifier on just the object region. Its fake training data are given by the $s''$ samples while its real inputs are given by $i' = i\circ m + i\circ(1-\b)$. As before, we add a feature matching loss $\calL^O_\text{\emph{FM}}$ using feature representations from $D_{O}$.

% Following previous GAN losses, we train $D_{O}$ and $G_I$:
% \begin{align}
%     % \calL_{D_{f}}(\Theta_{D_{f}}) &= -\E_{\z \sim \mathcal{N}(0,\,1), m\in \M, i\in \I}(\min(0, -D_{f}(s', m)-1)) - \E_{m\in \M, i\in \I}(\min(0, D_{f}(i,m)-1)), \nonumber \\
%     \calL_{D_{O}}(\Theta_{D_{O}}) = &-\E_{m\in \M, i\in \I}\Big(\E_{\z \sim \mathcal{N}(0,\,I)}(\min(0, -D_{O}(s'')-1)) + \min(0, D_{O}(i')-1)\Big), \nonumber \\
%     \calL^O_{G_{I}}(\Theta_{G_{I}}) = &-\E_{\z \sim \mathcal{N}(0,\,1), m\in \M, i\in \I}(D_{O}(s'')). \\
%     % \label{eq:hingeLSGAN}
%      \textbf{Final loss: } 
%     \calL(\Theta_{G_M}, \Theta_{D_M}, &\Theta_{G_{I}}, \Theta_{D_{I}}, \Theta_{D_{O}}) = \calL_{G_M} + \calL_{D_M} + \calL_{G_I} + \calL_{D_I}+\calL^O_{G_I} + \calL_{D_{O}} \nonumber \\
%      & + \lambda_1\cdot\calL^M_{rec} + \lambda_2\cdot\calL^O_{rec} + \lambda_3\cdot\calL^M_\text{\emph{FM}} + \lambda_4\cdot\calL^I_\text{\emph{FM}} + \lambda_5\cdot\calL^O_\text{\emph{FM}}.
% \end{align}

% Note that in this case we do not concatenate with the masks in the input to $D_{f^*}$ as 1) the main reason this was done in the beginning is still covered by $D_f$, 2) since the generated mask is already reflected in $s''$ then additionally concatenating to the input of $D_{f^*}$ makes it redundant. 
% \begin{align}
%     \calL^*_\text{\emph{FM}}(\Theta_{G_{f}}) = \sum_{l=1}^{L} \E_{\z \sim \mathcal{N}(0,\,1), m\in \M, i\in \I}( \|D_{f^*}^l(s'')- \bar{d_{f^*}^l} \|_2^2).
%     \label{eq:FM_loss*} 
% \end{align}
%\paragraph{Final loss:} 
%\begin{align}
%    \label{e:totalloss}
%    \calL(\Theta_{G_M}, \Theta_{D_M}, \Theta_{G_{I}}, \Theta_{D_{I}}, \Theta_{D_{O}}) =&  \calL_{G_M} + \calL_{D_M} + \calL_{G_I} + \calL_{D_I} + \calL^O_{G_I} + \calL_{D_{O}} + \nonumber \\
%    & \lambda_1\cdot\calL^M_{rec} + \lambda_2\cdot\calL^O_{rec} + \lambda_3\cdot\calL^M_\text{\emph{FM}} + \lambda_4\cdot\calL^I_\text{\emph{FM}} + \lambda_5\cdot\calL^O_\text{\emph{FM}}. \nonumber
%\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Attic
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Our goal is to sample realistic masks conditioned on a given background and bounding box location. 
% Our assumption is two folds, 1) The bounding box location substantially reduces the set of possible generated masks, 2) the background scene also reduces the set of possible masks, as it defines how the generated object should interact with its environment.
% We assume that combining these two inputs with a latent vector $\z_m \sim \mathcal{N}(0,\,1)$ can sample multiple realistic shapes and poses given annotated masks from a given object class. \ow{not sure we really need this paragraph} \jt{I also don't know what the point is.}

%\paragraph{Discussion:}
% each with varying object pose, object count, background, \etc~sampled from the respective domains $\S$ and $\T$. 
% Further, assume that each source image $\s \in \S$ is provided with an object segmentation mask $\s_{\m}\in\S_{\m}$. 
% Our goal is to learn a transfer function $f:\S\times\S_{\m}\to \T$ which translates objects in a source image $\s$ into objects in the target domain $\T$ in an output image $\mathbf{t}':=f(\s,\s_{\m})$.
% % We begin with source and target domains $\S,\T$ sampled as databases $S$ and $T$ of images of two object classes, each with varying object pose, object number, background, and so on. Given an image paired with its object segmentation mask $(\s, \s_{\m})$, our goal is to approximate a function $f$ such that $f(\s, \s_{\m}) = \mathbf{t}' \in \T$. 
% Figure \ref{fig:architecture} (left) visualizes our approach, as it relates to InstaGAN~\cite{instagan} (middle).

% %We may obtain $\mathbf{t}'$ using an auto-encoder; however, we wish to incorporate information from the segmentation mask in the decoding process. 
% As in InstaGAN~\cite{instagan}, we encode both $\s$ and $\s_{\m}$: $h_{\s} = \mathrm{enc}_\S(\s)$ and $h_{\s_{m}} = \mathrm{enc}_{\S_\M}(\s_{\m})$. Then, we concatenate these feature representations channel-wise and feed them: 1) into a decoder $\mathrm{dec}_\T$ which gives us $\mathbf{\hat{t}}'$, and 2) into a mask decoder $\mathrm{dec}_{\T_\M}$ which gives us $\mathbf{t}'_{\m}$.
% Formally this is expressed via $\mathbf{\hat{t}}' = G_\S(h_{\s}, h_{\s_{\m}})$, and $\mathbf{t}'_{\m}= G_{\S_\M}(h_{\s}, h_{\m_{\s}})$. Finally we obtain $\mathbf{t}'$ by feeding $\mathbf{\hat{t}}'$ to our differentiable blending module: $\mathbf{t}' = \text{Poissonblend}(\mathbf{\s, \hat{t}}', \s_{\m}, \mathbf{t}'_{\m})$. \ow{still refers to B} \ym{It is the same as the diagram now}

% To constrain our final results to look realistic, we use an adversarial discriminator $\D_\S$ which distinguishes between real pairs $(\s, \s_{\m})$ and fake pairs $(\mathbf{s}', \s'_m)$, where $\s'$ is the generated image from $\mathbf{t}\in\T$ (likewise for $\s'_{\m}$).
% The RGB and mask inputs are fed to the discriminator by first separately encoding them: $d_{\s} = \mathrm{enc}_{D_\S}(\s)$ and $d_{\s_{\m}} = \mathrm{enc}_{D_{\S_\M}}(\s_{\m})$. Then, similar to the generation part, we concatenate these feature representations channel-wise and feed them into a discriminator:
% $D_\S(d_{\s}, d_{\s_{\m}})$ gives us the probability of the pair $(\s, \s_{m})$ being real.


% In sum, we train an separate encoders for $\S$, $\S_\M$, $\T$, $\T_\M$, separate decoders for $\S$, $\S_\M$, $\T$, $\T_\M$, and separate discriminator encoders for $\D_\S$, $\D_{\S_\M}$, $\D_\T$, $\D_{\T_\M}$. 
% Their parameters are updated by playing the mini-max game governed by the Least Square GAN loss: 
% \begin{align}
%     \calL_\text{\emph{GAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) =& (D_\S(d_{\s}, d_{\s_{\m}}) -1)^2 +  \nonumber \\
%     &  (D_\T(d_{\mathbf{t}}, d_{\mathbf{t}_{\m}}) -1)^2 + \nonumber \\
%     & D_\S(d_{\mathbf{t}'}, d_{\mathbf{t}'_{m}})^2 + D_\T(d_{\s'}, d_{\s'_{m}})^2,
%     \label{eq:LSGAN}
% \end{align}
% where $\Theta_{D}$ contains the parameters of $D_\S, D_\T, D_{\S_\M}, D_{\T_\M}$, and $\Theta_{S}$ and $\Theta_{T}$ contain parameters of the encoding and decoding parts in $\S$, $\S_\M$ and $\T$, $\T_\M$ respectively.

%The system is joined cyclically such that all components involved in translations are trained simultaneously (Figure~\ref{fig:architecture}). Please see our supplemental material for details on the encoder and decoder architectures.


% \paragraph{Identity loss.}
% We also find that assisting the GAN objective with an identity loss, is necessary for convergence. Such loss  encourages the generated images to be identical to the inputs in the case where source and target domains are the same: \ym{Do we do that for both the mask and RGB or only RGB?}
% \begin{align}
%     \calL_{idt}(\Theta_{S}, \Theta_{T}) = \calL_{id}(\Theta_{S}, \Theta_{T}) + \calL_{id_{\m}}(\Theta_{S}, \Theta_{T}), 
% \end{align}
% such that:
% \begin{align}
%     \calL_{id}(\Theta_{S}, \Theta_{T}) =& \|\s -  G_\T(h_{\s}, h_{\s_{\m}})\|_1 + \nonumber \\  
%     &\|\mathbf{t} -  G_\S(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1, \nonumber\\
%     \calL_{id_{\m}}(\Theta_{S}, \Theta_{T}) =& \|\s_{\m} -  G_{\T_\M}(h_{\s}, h_{\s_{\m}})\|_1 + \nonumber \\
%     & \|\mathbf{t}_{\m} -  G_{\S_\M}(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1. \nonumber
% \end{align}

% Our final objective is hence written as: 
% \begin{align}
%     \calL(\Theta_{D}, \Theta_{S}, \Theta_{T}) = \calL_\text{\emph{GAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) + \lambda \calL_{idt}(\Theta_{S}, \Theta_{T}),
% \end{align}
% where $\lambda$ is a hyper-parameter that we fix to 10 \ym{check this}.

%We take lessons from InstaGAN’s use of segmentations and note that we can extend their use even further. 
%The segmentation masks provides us with not only the shape of the object but also its location. 
% We take advantage of the fact that the segmentations already define the areas of the image which need to be changed. Thus, we simply task our generator with creating a new foreground by “giving it” the background. We accomplish this by using a differentiable Poisson blend to restrict the output of our generator to the portion of it that lies within the. We slightly dilate the mask used to blend to allow our image generator how to modify areas around the foreground to make the blending more seamless.

% \paragraph{Poisson Blending Module}
% \ow{This part should be integrated into the above section. Instead of describing 1. instagan setup, then 2. our modifications, let's define 1. our architecture, and make sure we mention the similarity to instagan (and the differneces (missing loss fns)}
%Our Poisson module tasks the generator only to produce a new foreground while discarding the background. 
%Such behavior is possible by blending the newly generated foreground with the input background using the differentiable poisson blending algorithm described below. 
% From the discriminator point of view, it receives a generated image with a realistic background and a generated foreground. This encourages the generator to perfect its foreground generation in order for the mini-max game to converge.

% We build upon Farbman et al.'s convolution pyramid~\cite{farbman2011convolution} approximation of Poisson Blending~\cite{perez2003poisson}.
% The goal of this work is to reconstruct the image from its gradient field, where in Poisson Blending, the gradient field is composed of the foreground gradient composited onto the background gradient in the hole region.
% Poisson Blending involves finding a smooth ``membrane'' that interpolate of boundary colors on the hole by solving the Laplace equation. 
% This is computationally expensive, and convolution pyramids approximate it with an approximation of Shepard's ~\cite{shepard1968two} data interpolation method. 
%Shepard's
%Given a binary mask $\mathbf{m}$, a source image $\mathbf{s}$ and a target image $\mathbf{t}$, we first compute the mask boundary $\mathbf{b}$ by convolving $\mathbf{m}$ with a filter of size $3\times3$: $\mathbf{l} = [[0,-1,0],[-1,4,-1],[0,-1,0]]$. 
%Such filter, when convoluted on a region containing the same values, returns 0. Hence, when applied on the binary mask, $b=\mathbf{m}*\mathbf{l}$, only the boundary region will have non zero values. 
% \ow{I think we should actually put as little info as possible, as it is not our contribution, but that of convolution pyramids. I commented out the following section, but please check to see if you agree} \ym{Sounds good, I have put the maximum info possible as we can always truncate.}
%Shepard uses $\mathbf{b}$ to alter the source image via $\mathbf{s}'  =  \mathbf{s} + \mathbf{d}$, and $\mathbf{d}$ can be efficiently computed via: 
% \begin{align}
%     \mathbf{d}(x_i) = \frac{\sum_{j=0}^n d(x_i, x_j)\hat{b}(x_j)}{\sum_{j=0}^n d(x_i, x_j){b}(x_j)},
%     \label{eq:Shepard's}
% \end{align}
% where $d$ is a function that is inversely proportional to the distance between its inputs, $\hat b = b.(\mathbf{t} - \mathbf{s})$, and $n$ is the number of elements inside the mask. Note that, if $x_i$ is far away from the boundary then $d(x_i, x_j)$ will be close to zero. Meaning that $\mathbf{d}$ contains mostly zeros apart from the membrane surrounding the mask boundary, 
% which will contain values correcting the distribution shift in the source image compared to the target one. 

% Eq.~\ref{eq:Shepard's} is however not the most efficient, especially in our scenario where we are interested in reducing the computational cost of Image-to-Image translation. As such, Eq.~\ref{eq:Shepard's} can be seen as a ratio of convolutions that we approximate using convolutional pyramids~\cite{farbman2011convolution}. 

% Given an input $b$, we construct the convolutional pyramid output by first choosing the number of levels $L$ in the pyramid, then we feed the input to $L$ consecutive strided convolutions with a fixed kernel $h_1$, which performs the convolution operations while reducing the resolution of the input by half, formally this is expressed via: $b^{l+1} = \text{conv}(b^l, h_1)$, where the convolution here is computed using a stride of 2. 
% Then we compute the up-sampling pass by: $\hat b^{l} = \text{deconv}(\hat b^{l+1}, h_2) + \text{conv}(g, b^l)$, where $h_2$ and $g$ are both fixed kernels, with $\hat b^{L+1} = 0$. 
% The fixed kernels $h_1$, $h_2$ and $g$ are obtained by minimizing the $L_2$ norm between the output of the convolution pyramid and the desired linear transformation we wish to approximate, in our case Eq.~\ref{eq:Shepard's}. 
% Note that as a result of the numerical optimization, the kernels obtained are generalizable. In other terms they can be used on new images that have not been seen on the training set.

% By using such approach we can approximate the denominator and nominator of Eq.~\ref{eq:Shepard's} in linear time with respect to $n$, making our mappings from source to target and inversely run with minimal computations added compared to the vanilla GAN algorithm. 
% Most importantly, the convolutional pyramid used is fully differentiable which makes backpropagating through our network possible, This allows us to train with classical gradient based optimizers such as ADAM.

% The combination of real backgrounds and generated foregrounds as input to the discriminator is performed by blending the output of the generator to its input using as a mask the union of the real and generated foregrounds. The blending is an approximation of the well known Poisson blending using the previously discussed differentiable convolutional pyramids.


% \subsection{Simplified Objective Function}

% \vspace{.2cm}\noindent \textbf{Function.}

% \begin{align}
%     \calL_\text{\emph{GAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) =& (D_\S(d_{\s}, d_{\s_{\m}}) -1)^2 +  \nonumber \\
%     &  (D_\T(d_{\mathbf{t}}, d_{\mathbf{t}_{\m}}) -1)^2 + \nonumber \\
%     & D_\S(d_{\mathbf{t}'}, d_{\mathbf{t}'_{m}})^2 + D_\T(d_{\s'}, d_{\s'_{m}})^2,
%     \label{e:LSGAN}
% \end{align}
% where $\Theta_{D}$ contains the parameters of $D_\S, D_\T, D_{\S_\M}, D_{\T_\M}$, and $\Theta_{S}$ and $\Theta_{T}$ contain parameters of the encoding and decoding parts in $\S$, $\S_\M$ and $\T$, $\T_\M$ respectively.

% Note that compared to most of the image-to-image translation algorithms ~\cite{instagan, multimodal2018, almahairi2018augmented, yi2017dualgan}, our final loss function (Eq~\ref{eq:LSGAN}) is \emph{substantially} simplified, which allows our algorithm to train faster while focusing more on the GAN objective and hence, on the quality of generated images.
%Previous state of the art results have entailed cyclical loss functions~\cite{zhu2017unpaired}.
% While our training is entirely done by solely optimizing Eq.~\ref{eq:LSGAN}, the previous state of the art objectives~\cite{zhu2017unpaired,instagan}, are more complicated.
% Fig~\ref{fig:architecture} (middle) shows the InstaGAN architecture, consisting of the following loss functions:

% \begin{align}
%     \calL_\text{\emph{InstaGAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) =& \calL_\text{\emph{GAN}} + \lambda_1 * \calL_\text{\emph{idt}} +\nonumber\\
%     & \lambda_2 * \calL_\text{\emph{cycle}} + \lambda_3 * \calL_\text{\emph{ctx}},\nonumber
% \end{align}
% Where $\calL_\text{\emph{idt}}$ is an identity loss encouraging a generated images to be identical to itself in the case where source and target domains are the same:  

% \begin{align}
%     \calL_{idt}(\Theta_{S},\Theta_{T}) = \calL_{id}(\Theta_{S},\Theta_{T}) + \calL_{id_{\m}}(\Theta_{S},\Theta_{T}),\nonumber
% \end{align}
% with: 
% \begin{align}
%     \calL_{id}(\Theta_{S},\Theta_{T}) =& \|\s -  G_\T(h_{\s}, h_{\s_{\m}})\|_1 + \nonumber\\
%     &\|\mathbf{t} -  G_\S(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1, \nonumber
% \end{align}
% \begin{align}
%     \calL_{id_{\m}}(\Theta_{S},\Theta_{T}) =& \|\s_{\m} -  G_{\T_\M}(h_{\s}, h_{\s_{\m}})\|_1 + \\ &\|\mathbf{t}_{\m} -  G_{\S_\M}(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1.
% \end{align}
% and $\calL_{id_{\m}}$ serves the same purpose as $\calL_{id}(\Theta_{S},\Theta_{T})$ but applied on masks instead.

% Constraining the generation even further, the cyclic loss ensures that images are mapped to themselves when mapped from source to target and back to to source:  
% \begin{align}
%     &\calL_{cyclic}(\Theta_{S}, \Theta_{T}) = \calL_{cyc}(\Theta_{S},\Theta_{T}) +\calL_{cyc_{\m}}(\Theta_{S},\Theta_{T}), \nonumber\\
%     &\calL_{cyc}(\Theta_{S}, \Theta_{T}) = \| \s - \s''\|_1 + \| \mathbf{t} - \mathbf{t}''\|_1, \nonumber \\
%     &\calL_{cyc_{\m}}(\Theta_{S}, \Theta_{T}) = \| \s_{\m} - \s_{\m}''\|_1 + \| \mathbf{t}_{\m} - \mathbf{t}_{\m}''\|_1,\nonumber
% \end{align}
% where $\s'' = G_\T(h_{\s'}, h_{\s_{\m}'})$, with $h_{\s'} = E_\T(\s')$ and $h_{\s_{\m}'} = E_{\T_\M}(\s_{\m}')$. Likewise for $\s_{\m}''$.

% Finally, the \emph{context loss} enforces the \emph{intersection} of backgrounds in $\s_{\m}$ and $\mathbf{t}_{\m}'$ to not change: 
% \begin{align}
% \calL_{ctx}(\Theta_{S}, \Theta_{T}) =& \|(\s-\mathbf{t}') \odot w(\s_{\m}, \mathbf{t}_{\m}')\|_1  \nonumber + \\
% &\|(\mathbf{t}-\s') \odot w(\mathbf{t}_{\m}, \mathbf{s}_{m}')\|_1,
% \label{eq:ctx}
% \end{align}
% where $\odot$ represents Hadamard product and $w(\s_{\m}, \mathbf{t}_{\m}') =  1 - \max(\s_{\m}, \mathbf{t}_{\m}')$ . However since Eq.~\ref{eq:ctx} operates as a soft constraint, background changes and artifacts still occur as depicted in Fig.~\ref{tab:background_examples}.

% Removing the cycle consistency loss and the identity loss considerably decreases the computational overhead required to complete a forward pass, and emoving the context loss encourages the generator to focus only on the foreground generation.
% Using our differentiable blending module, we are left only the adversarial loss, similar to the original GAN proposed by Goodfellow et. al~\cite{goodfellow2014generative}.
% This has the added benefit of requiring fewer hyper-parameters to balance the different loss terms. 

%3) adding our differentiable blending module which simplifies the image-translation problem, enabling us to remove the previously discussed losses while improving the image quality.  

%\subsection{Advantages: Less is More}
% Our advantages over InstaGAN are threefold. Our approach: 
% \ag{Should this be 4?}
% \ms{Do you mean 4 contributions?}
% \begin{enumerate}
%     \item Halves the number of parameter updates required at each step of training through the removal of cyclic loss.
%     \item Removes the need for tuning hyperparameters for identity loss, cyclic loss and context loss.
%     \item Prevents the generator from:
%         \begin{enumerate}
%             \item reconstructing the background leading to compounding reconstruction error potential degradation of image quality.
%             \item reconstructing visual details that are lost during the translation. The generator no longer needs to wastefully steganographically encode this information~\cite{chu2017cyclesteg}. 
%         \end{enumerate}
% \end{enumerate}

%Our network does not require dataset specific tuning of these hyper parameters and is able to prevent background leakage with additional degrees of robustness. This simplicity makes our approach much more applicable to novice AI practitioners who may lack the domain knowledge and additional compute to train these models. 
% \ow{we need to show 1. the full loss function, and then 2. our reduced one, with clearly fewer terms.}

%We are able to abstract ourselves from InstaGANs losses and hence their hyperparameters by presenting the discriminator with images containing a generated foreground combined with a real background. This, in turn, encourages the generator to perfect its foreground generation and makes the image translation problem much simpler. Indeed, the generator's capacity is in this case not wasted on altering the background as an attempt to fool the discriminator but is solely devoted to generating a plausible foreground.  


% \paragraph{Sequential training:} As we are using object-centered datasets with mutilple instances, we use the same sequential training strategy as InstaGan. Given an image containing $n$ instances, we select their $n$ corresponding masks, then on each sequence iteration we feed the image and two masks to the generator until the $n$ masks are consumed. At the end of each iteration, we update the subsequent real image with the newly blended fake image.  If $n$ is odd, then we feed an empty mask alongside the final mask. 
% Fig~\ref{fig:architecture} (right), shows the sequential training strategy.
% The combination of real backgrounds and generated foregrounds as input to the discriminator is performed by blending the output of the generator to its input using as a mask the union of the real and generated foregrounds. The blending is an approximation of the well known poisson blending using the previously discussed differentiable convolutional pyramids.
% We wish to emphasize that our network architecture makes our generator mapping more restricted than other architectures. Our segmentation generator’s output is fed directly to the discriminator, so the regularization effects of the discriminator restrict the generator’s segmentations to realistic objects in the target domain. If the generator were to create abstract segmentations, it would be penalized.

% Since, our image generator may only modify areas within this segmentation, it does not attempt some of the strategies taken by generators of other architectures, such as contorting the background or changing the image’s lighting. Thus, we are able to remove the identity and cylic losses. 

% Our discriminators are also multi-scale, which has demonstrated better results on these tasks~\cite{Gokaslan2018, multimodal2018,Li2018UnsupervisedIT}.

% \paragraph{Cyclic loss.}
% Unpaired image translation is an under-constrained problem even with $\calL_\text{\emph{GAN}}$.
% To further constrain it, we adopt the Zhu et al.~\cite{zhu2017unpaired} cyclic consistency which helps conserve characteristics of the input image (\eg, the pose of the object).
% For this purpose, we could use a cycle energy loss on both the input images and their masks. This encourages an image mapped twice (from source to target to source) to be identical to the original image:
% \begin{align}
%     \calL_{cyc}(\Theta_{S}, \Theta_{T}) &= \| \s - \s''\|_1 + \| \mathbf{t} - \mathbf{t}''\|_1, \\
%     \calL_{cyc_{\m}}(\Theta_{S}, \Theta_{T}) &= \| \s_{\m} - \s_{\m}''\|_1 + \| \mathbf{t}_{\m} - \mathbf{t}_{\m}''\|_1,
% \end{align}
% where $\s'' = G_\T(h_{\s'}, h_{\s_{\m}'})$, with $h_{\s'} = E_\T(\s')$ and $h_{\s_{\m}'} = E_{\T_\M}(\s_{\m}')$. Likewise for $\s_{\m}''$. %\kimki{I guess the squared terms in the above equations are mistakes?}\ym{which squared terms? we followed the InstaGAN setting where the cycle energies are not squared.}\kimki{I mean, having the norm squared in the source domain terms but not in the target domain terms??} \ym{yup sorry you are right} \kimki{Thanks}

% While cyclic loss both aids the network in preventing mode collapse and in preserving attributes across domains, the term has limitations. The bijective constraint can hinder shape change~\cite{Gokaslan2018, zhu2017unpaired} and texture transfer. Small irrelevant details must be preserved to perfectly reconstruct the original image. Instead, we focus on reconstructing a much simpler task: the original segmentation. In our results, we will show empirically that minimizing only $ \calL_{cyc_{\m}}$ is enough to achieve the goal initially desired by cycle energies.

% We find that eliminating the RGB reconstruction loss improves the quality of generated images (Table~\ref{t:kid_ablation}). The remaining loss terms provide adequate stability to the network to prevent mode collapse. Furthermore, unlike previous methods which do not require cyclic reconstruction~\cite{benaim2017one}, our method can handle shape change.

%\begin{align}
%    \calL_{id} =& \|\s -  G_\T(h_{\s}, h_{\s_{\m}})\|_1 +  \nonumber \\ 
%    &\|\mathbf{t} -  G_\S(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1,
%\end{align}
%\begin{align}
%    \calL_{id_{\m}} =& \|\s_{\m} -  G_{\T_\M}(h_{\s}, h_{\s_{\m}})\|_1 +  \nonumber \\
%     &\|\mathbf{t}_{\m} -  G_{\S_\M}(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1.
%\end{align}
% \paragraph{Context loss.}
% Jointly optimizing the previous three losses enables shape change for image-to-image translation; however, there is no mechanism encouraging only foreground objects of interest to be altered, \eg, in the giraffe to sheep problem, one should be able to change a giraffe to the corresponding sheep without altering the background.
% One way to achieve such property is to enforce the initial background pixels in $\s$ and given by $\s_{\m}$ not to change in $\mathbf{t}'$.
% However, doing so would be in opposition with our initial motivation of performing significant shape changes across domains as, in that scenario, pixels which were initially in the background of $\s$ could end up being in the foreground of $\mathbf{t}'$.
% For this reason, we instead enforce the \emph{intersection} of backgrounds in $\s_{\m}$ and $\mathbf{t}_{\m}'$ not to change, which allows for shape change while encouraging the background to be conserved as in InstaGAN
% % \kimki{Can we remove `That is:' and finish the previous sentence as `to be conserved:'?} That is: %\jt{edited equations back}
% \begin{align}
% \calL_{ctx}(\Theta_{S}, \Theta_{T}) =& \|(\s-\mathbf{t}') \odot w(\s_{\m}, \mathbf{t}_{\m}')\|_1  \nonumber + \\
% &\|(\mathbf{t}-\s') \odot w(\mathbf{t}_{\m}, \mathbf{s}_{m}')\|_1,
% \end{align}
% where $\odot$ represents Hadamard product and $w(\s_{\m}, \mathbf{t}_{\m}') =  1 - \max(\tilde{\s}_{\m}, \tilde{\mathbf{t}}_{\m}')$ with $\tilde{\s}_{\m}$ being the binary, rounded version of the initial mask. Furthermore, since this constraint operates as a soft constraint, the network may make small changes outside the segmentation that enhance the plausibility of the image. For instance, filling gaps in between segmentation or slightly changing the lighting tone or vegetation in an image.

% \paragraph{Feature matching loss.} Finally, we define a feature matching loss which we find to encourage sharper and more realistic images. This loss encourages feature representations computed from $\{\mathbf{s}'_i\}_{i=1}^{N_t}$ to be close in terms of the $L2$ norm with respect to the features computed from $\{\mathbf{s}_i\}_{i=1}^{N_s}$, where $N_s$ and $N_t$ are the number of datapoints for domains $\S$ and $\T$ respectively. 
% %\kimki{Can we use the term L2 distance instead of Euclidean distance as we already used $\|\cdot\|_2$?}\kimki{What is $N$? The number of images? Can an image have multiple objects?}\ym{addressed}\ag{Can we fix the double subscript Latex issue?}\ym{which one, I thought this was solved as I dropped the i indices?} 
% Such feature representations are extracted in this case from $D_\S$. 

% This loss has been shown to help produce good generated images~\cite{salimans2016improved,wang2017pix2pixHD,Gokaslan2018,wang2018vid2vid}. The intuitive reason why this works is that we wish neurons in the source domain discriminator to be activated in the same way between generated source images and real ones. This ends up reinforcing the realism of the generator, $G_\S$ in this case.

% Formally, we express this via the following loss: 
% \begin{align}
%     \calL_{FM}(\Theta_{S}, \Theta_{T}) = \sum_{l=1}^{L-1} &\E_{\s \sim B}(\|D_\S^l(\s') - D_\S^l(\mathbf{s})\|_2^2) + \nonumber \\ 
%     &\E_{\mathbf{t} \sim B}(\|D_\T^l(\mathbf{t}') - D_\T^l(\mathbf{t})\|_2^2), \label{eq:FM}
% \end{align}
% %\kimki{A quick question: the expectations above are just sums over data points within the mini-batch $B$. Is it correct?}\ym{Indeed}\kimki{Thanks. Summation might be easier to understand than this mathematically ill-defined expectation symbol in this case. But this notation is well-established :(.}
% where $L$ is the number of layers in the discriminator architecture, $B$ is the mini-batch, and $D^l$ is the feature activation of the corresponding discriminator at layer $l$. Moreover, since we use a small batch size, directly enforcing Eq.~\ref{eq:FM} %
% %Eq.~\eqref{eq:FM} 
% may be less valid for a given pair of $s_i'$ and $s_i$. We introduce the novel contribution of maintaining an exponential moving average for feature representations of the real images and use them instead in Eq.~\ref{eq:FM}. 

 

% \paragraph{InstaGAN3D:}
%  this model builds upon InstaGAN and improves it by adding two adversaries, the first discriminates between real and generated segmentation masks, while the second discriminates between real and generated images.  
%  Trained jointly with the initial discriminator, we find that doing so encourages sharper generated images, see Figure.


% Our work is inspired by recent works such as ContrastGAN~\cite{liang2017} and InstaGAN~\cite{instagan} which augment CycleGAN with a segmentation map. We make several important changes, each of which meaningfully improves the translation quality as we show in the ablation study (Sec.~\ref{s:results}). For clarity, we list all changes below.

% \vspace{.2cm}\noindent \textbf{Additions.}
% Over losses in InstaGAN, we add relativistic average discriminators~\cite{jolicoeurRelativistic} via least squares GAN~\cite{mao2017least}, multi-scale discriminators, and feature matching loss. We also maintain an exponential moving average over the feature match loss to learn the feature statistics of real images across the entire dataset despite the small minibatch size.

% \vspace{.2cm}\noindent \textbf{Subtractions.}
% We remove the `\emph{insta}nce' from InstaGAN: We only provide one mask per image which contains the intersection of all per-instance masks, instead of one mask per instance in the image framed as recursive segmentation. This reduces complexity and avoids the need for expensive explicit instance segmentation. We show that this still achieves high quality results. Further, we do not enforce a cyclic loss on the RGB reconstruction and only on the mask reconstruction, which again saves computation.



%minimizing the cycle loss energy with respect to real and generated images can prevent shape change as CycleGAN~\cite{zhu2017unpaired} demonstrates. 
%InstaGAN manages to counter this effect by using additional supervision, however minimizing the cycle energy in that way, forces the generator to smartly hide source domain information (e.g. the neck of a Giraffe) by partly in-painting them (See Figure\ref{}), which produces artifacts on the final result.
 %We reduce this effect by enforcing a weaker cycle energy that only acts on the masks (i.e we only reconstruct the masks). Doing so, removes the burden of reconstructing textures while encourages properties such as the pose to be conserved.



==> src/3-method_backup.tex <==
\section{Method}
\label{sec:Method}
\zs{For an input image $i\in\mathcal{I}$, given the user-drawn bounding box $b$ with a given class $c$, our goal is to synthesize a stamped image $i_{\hat{s}}$ by combining a generated stamp object image $\hat{s}$ and $i$. The stamp $\hat{s}$ should be seamlessly incorporated into $i$ such that $i_{\hat{s}}$ cannot be discriminated from the images in $\mathcal{I}$.}
\kimki{Do we need hat ($\hat{s}$) for $s$?}\zs{Since the stamp is generated by our model, I'd like to use hat to differentiate from the ground truth. } \kimki{An alternative to the next sentence: ``As constructing a network that generates such stamps is a seriously ill-posed problem, we stratify its training by decomposing it into two phases and provide the corresponding intermediate level supervision.''} \zs{To achieve high-quality outputs, we decouple the generation of shape and texture of $\hat{s}$ for better injecting supervision information. As a result, there are two steps in the proposed method, namely, 1) stamp shape mask generation and 2) stamp texture generation. They are both conditional generation, and the generators are trained in an adversarial fashion. Fig.~\ref{fig:architecture} shows the overview of our architecture, and we will explain them in detail in the subsequent sections.}
Our method consists of two steps: learning to synthesize object shapes from a database of binary masks $\M$, and learning to synthesize object texture from a corresponding database of images $\I$ (Fig.~\ref{fig:architecture}). Architecture details for all networks are provided in the supplementary material.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning to synthesize object shapes\zs{Learning to synthesize stamp shapes}} 
%%%%%%%%%%%%
% Variables & naming
%
% \I = database of images
% \M = database of masks
% i = an image
% m = a mask

% D = discriminator
% G = generator
% G_I, G_M, D_I, D_M = image/mask generators/discriminators

% b = bounding box
% \z_m = random latent vector used per sample (is that right? is z per sample?)
% |\z_m| = number of entries in z_m; saves introducing n

% \Theta = network parameters

\zs{The stamp shape mask generation model $G_M$ is a conditional-GAN. It takes a processed image $i_b$ as an input and outputs a binary mask $\hat{m}$ for the shape of the stamp object: $\hat{m} = G_M(i_b, z_m)$ ($z_m$ is the random vector for GAN). For $i_b \in R^{ H\times W\times 3}$, it contains part of $i$ excluding the box region $b$. The content of $i$ in region outside user-input box $b$ is preserved, while that inside $b$ is discarded and set to 0. For $\hat{m}\in R^{ H\times W\times 1}$, the tensor is real-valued between 0 and 1, where 1 denotes shape region while 0 denotes the background.}\kimki{I would suggest try not to use terms specific to a software package.}

We wish to train a network $G_M$ to generate an object mask (real valued; $[0,1]$) which fools a discriminator $D_M$. Given a training database image $i \in \I$ containing at least one instance of a given class, \kimki{CVPR recommends \eg over `e.g.':} e.g., `giraffe', we randomly pick an instance. Given its binary mask $m \in \M$, we create a vector $b$ which describes the bounding box location of the object: if $[x_1, y_1]$ and $[x_2, y_2]$ are the top left and bottom right coordinates, and $h$ and $w$ are the height and width of the image, then $b = [\frac{x_1}{h}, \frac{y_1}{w}, \frac{x_2}{h}, \frac{y_2}{w}]$. 
Next, we form the background conditioning image $i_c$ by setting the region within the bounding box (containing the giraffe) to black. 
Further, to learn to generate diverse examples via stochasticity, we condition mask generation on a randomly sampled latent variable $\z_m$. 


We pass $i_c$ as input to $G_M$, and we inject $b$ and $\z_m$ into $G_M$ via adaptive instance normalization (AdaIN)~\cite{huang2017adain}.
Specifically, we concatenate $b$ and $\z_m$ into a conditioning vector, then we pass this through a Multi-Layer Perceptron (MLP) which predicts the parameters of an affine transformation applied to the Instance Normalization layers. 
This approach has seen success in style transfer applications~\cite{huang2017adain, multimodal2018,karras2018style,romero2018smit}. 
However, $b$ and $\z_m$ could be ignored: na\"{i}ve injection does not ensure that the generated mask will be wholly contained within the user-defined bounding box, nor that the mapping will be stochastic.

To preserve the bounding box constraints, we condition our mask discriminator network $D_M$ on $b$: we tile the vector $b$ into a $w\times h \times 4$ array and concatenate it with $m$.
This ensures that the generated masks are realistic, and that they agree with $b$ in the same way that real masks agree with $b$.

To preserve mask stochasticity, we use a reconstruction loss on $\z_m$:
% \kimki{(with $|\z_m|$ being the dimensionality of $\z_m$)}:
\begin{align}
    \calL^M_{rec}(\Theta_{G_{M}}) = \frac{1}{|\z_m|} \left\| \z_m - \text{Enc}_m( \text{MLP}(\z_m, b))\right \|_1^2,
    \label{eq:maskzrecloss}
\end{align}
where $\Theta_{G_{M}}$ are the learnable parameters of $G_M$, $\text{MLP}$ predicts the affine parameters of the AdaIN layers, and $\text{Enc}_m$ is a fully-connected encoder trained to reconstruct $\z_m$. 
In contrast to other algorithms~\cite{multimodal2018,zhu2017bicycle}, we do not reconstruct $\z_m$ from the image but rather \emph{directly} from $\text{MLP}(\z_m,b)$ as we find it to give better results.
It is not easy for the network to ignore variance in AdaIN parameters, and this approach essentially forces the AdaIN parameters to vary with respect to $\z_m$.


We train $D_M$ and $G_M$ using the hinge-GAN loss, which is known for its training stability \cite{lim2017geometric,tran2017deep,miyato2018spectral}:\kimki{Can we use $\mathbb{E}$ instead of $\mathcal{E}$ to denote an expectation?}
\begin{align}
    \calL_{D_M}&(\Theta_{D_M}) = \\
               &-\E_{\z_m \sim \mathcal{N}(0,\,I)}(\min(0, -D_M(m', b)-1)) \nonumber \\
               &-\E_{m\in \M}(\min(0, D_M(m,b)-1)), \nonumber \\
    \calL_{G_M}&(\Theta_{G_M}) = -\E_{\z_m \sim \mathcal{N}(0,\,I)}(D_M(m', b)),
\label{eq:hingeLSGANmask}
\end{align}
where $m'=G_M(i_c, \z_m, b)$ is the generated mask (real values in $[0,1]$), and $\Theta$ is the respective set of network parameters. \kimki{``and $\mathcal{N}(0,I)$ denotes the standard normal distribution.''} \kimki{What don't we use $\mathcal{N}$ (instead of $\mathcal{N}(0,1)$) and define it as the standard normal distribution?}

Furthermore, we enhanced the perceived quality of the reconstructed image by adopting the deep feature matching loss~\cite{salimans2016improved,zhang2018unreasonable}.
Such a loss enforces that the real and generated images produce similar feature responses in terms of the squared $L_2$ norm on each layer of the discriminator: 
\begin{align}
    \calL^M_\text{\emph{FM}}(\Theta_{G_M}) = \sum_{l=1}^{L_{D_M}} \E_{\z_m \sim \mathcal{N}(0,\,I)}( \left\|D_M^l(m', b)- \bar{d}^l_m \right\|_2^2),
    \label{eq:maskFM_loss} 
\end{align}
where $L_{D_M}$ is the number of layers in $D_M$ and $\bar{d}^l_m$ is the moving average at layer $l$ of $D_M^l(m,b)$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning to synthesize object texture}
We can now generate realistic masks conditioned on a user's bounding box and background image. Our next goal is to texture the mask.
To do this, we train an object texture generator $G_{I}$ using a general image adversary network $D_{I}$, which is trained as a real/fake classifier assessing the quality of both the generated texture as well as how it blends with the background.
%Inspired by Zhu et al's bicycle GAN~\cite{zhu2017bicycle} and 
% Both are trained as a real/fake classifiers and see real object instances, with $D_I$ seeing them against real backgrounds.
In addition, we want to enforce stochastic texture generation to represent variation in object appearance. 

Given a real image $i \in \I$ and a mask $m \in \M$ for a single object instance in $i$, the input to the generator $G_{I}$ is the masked real background $s = i\circ(1-m)$, where $\circ$ is the element-wise product, and a latent vector $\z_i$ to enforce stochasticity in the texture generation. 
$\z_i$ is concatenated layer-wise into the encoding part of $G_{I}$. Similar to Eq.\ref{eq:maskzrecloss}, we encourage a stochastic texture generation process via a latent reconstruction loss $\calL^I_{rec}$ on $\z_i$:
\begin{align}
    \calL^z_{rec}(\Theta_{G_{I}}, \z_i) = \frac{1}{|\z_i|} \left\|\z_i - \text{Enc}(s'\circ m)\right\|_1^2.
    \label{eq:zrec}
\end{align}

In Eq.~\ref{eq:zrec} and following~\cite{zhu2017bicycle}, we reconstruct the latent vector from the generated foreground $s'\circ m$. 
%
We then create a composite image $s'$ from the element-wise sum of generated object and real background:
\begin{align}
    s' &= G_{I}(s, \z_i) \circ m + i \circ (1-m).
    \label{eq:s'}
\end{align}

To improve the details in our generated images we impose a set of reconstruction and feature matching losses. First we use a pixel-wise reconstruction loss: 
\begin{align}
    %\calL^i_{rec}(\Theta_{G_{I}}, s') = \frac{1}{\left\|m\right\|_0} \left\|i - s'\right\|_1^2,
    \calL^i_{rec}(\Theta_{G_{I}}, s') = \frac{\|i - s'\|_1^2}{\|m\|_0},
    \label{eq:irec}
\end{align}
where we normalize by the sum of non zero elements in $m$ to equally account for instances of different sizes. 
 When doing so, Eqs.~\ref{eq:zrec},~\ref{eq:irec} \kimki{``serve contradictory purposes''?} are in direct opposition.have a contradictory purpose.
 Indeed, doing so encourages our network to reconstruct $i$ from a random latent vector $z_i$ that differs from an epoch to the other. 
 
To account for this, we use an additional latent vector $\z'_i$, which we obtain by encoding the real foreground: $\text{Enc}(i \circ m)=\z'_i$. Then, using~\ref{eq:s'} and $\z'_i$, we generate the image $s''$ which is applied as input to Eq.~\ref{eq:irec} instead of $s'$. 
\ow{clarify these last two paragraphs, I don't get the point}

We find that adding a perceptual loss~\cite{johnson2016perceptual} helps recreate fine textural details, e.g. the tail of the giraffes in Fig~\ref{}.
This loss uses a pre-trained VGG16 network to extract features for two image instances, then enforces their feature activations to be as similar as possible. In our case we use the features from the third hidden layer: 
\begin{align}
    \calL^i_{p}(\Theta_{p}, i, s'') = \frac{1}{N} \left\|\phi(i) - \phi(s'')\right\|_1^2,
    \label{eq:irec2}
\end{align}
where $\phi(i)$ are extracted features of $i$, and $N$ its cardinal. 

We facilitate the sampling at test time and we avoid large values in $z'_i$ by enforcing it to be sampled from a random normal distribution. 
We achieve this by using the re-parametrization trick~\cite{kingma2013auto} on $\text{Enc}$, then we add a KL loss between $z'_i$ and a randomly sampled vector $q\sim \mathcal{N}(0,\,I)$ of the same shape.


The inputs to the discriminator $D_{I}$ are the channel-wise concatenation of the real tuple $(i,m)$, and the fake image tuple $(s',m)$. It might seem like $D_{I}$ should only need to see $i$ or $s'$ to tell whether an object has been realistically textured against a background. However, without $m$, our generator will eventually learn to texture the object mask \emph{with background} because some database images contain multiple object instances: Suppose there are two giraffes in an image, and our generator must learn to texture the first giraffe mask. The generator could place background-like texture, which is easier, and $D_{I}$ would \emph{still be satisfied} that the image is real by its observation of the second giraffe instance. Explicitly forcing $D_{I}$ to observe only giraffe regions forces the generator to texture as desired.

For training, we adopt hinge-GAN-based losses using both $s'$ and $s''$:
{\small
\begin{align}
    \calL_{D_{I}}&(\Theta_{D_{I}}) = \\
                 &-\E_{m\in \M, i \in \I}\big(\E_{\z_i \sim \mathcal{N}(0,\,I)}(\min(0, -D_{I}(s', m)-1)) \nonumber \\ 
                 & + \E_{\z'_i}(\min(0, -D_{I}(s'', m)-1)) \nonumber \\ 
                 &+ \min(0, D_{I}(i,m)-1)\big), \nonumber \\
    \calL_{G_{I}}&(\Theta_{G_{I}}) = \\
                 &-\E_{\z \sim \mathcal{N}(0,\,I), m\in \M, i\in \I, \z'_i}(D_I(s', m) + D_I(s'', m)) \nonumber,\\
    \label{eq:hingeLSGANgt}
\end{align}
}%
\kimki{Shouldn't $\E_{m\in \M, i \in \I}$ be a summation?: $\sum_{m\in \M, i \in \I}$;} \kimki{I guess in the second summand, the expectation should be written as $\E_{\z_i \sim \mathcal{N}(0,I)}$?}
where $\Theta_{D_{I}}$ and $\Theta_{G_{I}}$ are network parameters of $D_{I}$ and $G_{I}$ respectively. Similar to the mask generation step (Eq.~\ref{eq:maskFM_loss}), we also use a deep feature matching loss $\calL^I_\text{\emph{FM}}$, but since we have the ground truth image $i$, we do not use feature moving averages:
{\small
\begin{align}
    %\calL^I_\text{\emph{FM}}&(\Theta_{G_{I}}) = \\
     %&\sum_{l=1}^{L_{D_I}} \E_{\z'_i, m\in \M, i\in \I}\left( \left\|D_{I}^l(s'', m)- D_{I}^l(i, m) \right\|_1^2\right). \nonumber\\
     \calL^I_\text{\emph{FM}}&(\Theta_{G_{I}}) = \\
     &\sum_{l=1}^{L_{D_I}} \E_{\z'_i, m\in \M, i\in \I}\left(\|D_{I}^l(s'', m)- D_{I}^l(i, m) \|_1^2\right). \nonumber\\
    \label{eq:FM_loss} 
\end{align}
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Simultaneous generator training} 
% To allow us to train both the object mask $G_{M}$ and texture $G_{I}$ generators together, we construct $s$, the input to $G_I$, using the generated mask $m'$: $s = i\circ(1-m')$. This approach creates a gradient flow between $G_{M}$ and $G_{I}$ during training, i.e., as mask realism increases it has a potentially positive effect on texture realism. This also helps ensure that the synthesized masks $m'$ at testing do not significantly deviate from the training masks $m$.

%Again, we encourage the adversarial and feature matching losses alone in that stage does not encourage a stochastic texture generation. Indeed, if the generator ignores $z^*$ then it is still possible to minimize Eqs~\ref{eq:hingeLSGANgt},~\ref{eq:FM_loss*}. To avoid this situation we add a latent reconstruction loss on $z^*$, which enforces that the information carried in it does not get ignored:

% where $\text{MLP}$ is the Multi-Layer Perceptron used to predict the affine parameters of ADAIN layers and $\text{Enc}$ is a fully connected encoder whose job is to reconstruct $z^*$, and $n_{z^*}$ is the number of elements in $z^*$ which is set 20. Note that in contrast with other existing algorithms, we do not reconstruct $z^*$ from the image but rather directly from $\text{MLP}(z^*)$ as we find it to empirically give better results.  

% We obtain the image to be fed to the discriminator $D_I$ as:
% \begin{align}
%     %s'' = G_I(s, \z_i^*)\circ m' + i\circ (1-\b),
%     s'' = G_I(s, \z_i)\circ m' + i\circ (1-\b),
%     \label{eq:s''}
% \end{align}
% where $\b$ is a 2D binary mask where pixels inside the coordinates of $b$ are 1 and outside are 0. 

% Eq.~\ref{eq:s''} is different from the equivalent operation on real inputs, as defined in Eq.~\ref{eq:s'}. In Eq.~\ref{eq:s'}, we use all of the real background outside the mask, while in Eq.~\ref{eq:s''} we only use the background given by $i\circ(1-\b)$. This is because at training time $b$ \emph{already contains} an instance, and so replacing the background by $i\circ(1-m')$ as in Eq.~\ref{eq:s'} might `overlay' or `merge' two instances inside $b$: the generated one and the original one. This unexpected signal distorts object appearance and disturbs training. Note that Eq.~\ref{eq:s''} is only applied at training time; at test time we use Eq.~\ref{eq:s'}.  

%\paragraph{Object discriminator:}
% \noindent\textbf{Object discriminator:}
% $s'$ and $s''$ have different content: $s'$ has complete background and object texture inside $b$, but $s''$ has no background texture inside $b$. Thus, we cannot use the same adversary $D_{I}$ to train the generator $G_I$ with respect to $s''$. Instead we introduce a new object discriminator $D_{O}$ which acts as a real/fake classifier on just the object region. Its fake training data are given by the $s''$ samples while its real inputs are given by $i' = i\circ m + i\circ(1-\b)$. As before, we add a feature matching loss $\calL^O_\text{\emph{FM}}$ using feature representations from $D_{O}$.

% Following previous GAN losses, we train $D_{O}$ and $G_I$:
% \begin{align}
%     % \calL_{D_{f}}(\Theta_{D_{f}}) &= -\E_{\z \sim \mathcal{N}(0,\,1), m\in \M, i\in \I}(\min(0, -D_{f}(s', m)-1)) - \E_{m\in \M, i\in \I}(\min(0, D_{f}(i,m)-1)), \nonumber \\
%     \calL_{D_{O}}(\Theta_{D_{O}}) = &-\E_{m\in \M, i\in \I}\Big(\E_{\z \sim \mathcal{N}(0,\,I)}(\min(0, -D_{O}(s'')-1)) + \min(0, D_{O}(i')-1)\Big), \nonumber \\
%     \calL^O_{G_{I}}(\Theta_{G_{I}}) = &-\E_{\z \sim \mathcal{N}(0,\,1), m\in \M, i\in \I}(D_{O}(s'')). \\
%     % \label{eq:hingeLSGAN}
%      \textbf{Final loss: } 
%     \calL(\Theta_{G_M}, \Theta_{D_M}, &\Theta_{G_{I}}, \Theta_{D_{I}}, \Theta_{D_{O}}) = \calL_{G_M} + \calL_{D_M} + \calL_{G_I} + \calL_{D_I}+\calL^O_{G_I} + \calL_{D_{O}} \nonumber \\
%      & + \lambda_1\cdot\calL^M_{rec} + \lambda_2\cdot\calL^O_{rec} + \lambda_3\cdot\calL^M_\text{\emph{FM}} + \lambda_4\cdot\calL^I_\text{\emph{FM}} + \lambda_5\cdot\calL^O_\text{\emph{FM}}.
% \end{align}

% Note that in this case we do not concatenate with the masks in the input to $D_{f^*}$ as 1) the main reason this was done in the beginning is still covered by $D_f$, 2) since the generated mask is already reflected in $s''$ then additionally concatenating to the input of $D_{f^*}$ makes it redundant. 
% \begin{align}
%     \calL^*_\text{\emph{FM}}(\Theta_{G_{f}}) = \sum_{l=1}^{L} \E_{\z \sim \mathcal{N}(0,\,1), m\in \M, i\in \I}( \|D_{f^*}^l(s'')- \bar{d_{f^*}^l} \|_2^2).
%     \label{eq:FM_loss*} 
% \end{align}
%\paragraph{Final loss:} 
%\begin{align}
%    \label{e:totalloss}
%    \calL(\Theta_{G_M}, \Theta_{D_M}, \Theta_{G_{I}}, \Theta_{D_{I}}, \Theta_{D_{O}}) =&  \calL_{G_M} + \calL_{D_M} + \calL_{G_I} + \calL_{D_I} + \calL^O_{G_I} + \calL_{D_{O}} + \nonumber \\
%    & \lambda_1\cdot\calL^M_{rec} + \lambda_2\cdot\calL^O_{rec} + \lambda_3\cdot\calL^M_\text{\emph{FM}} + \lambda_4\cdot\calL^I_\text{\emph{FM}} + \lambda_5\cdot\calL^O_\text{\emph{FM}}. \nonumber
%\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Attic
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Our goal is to sample realistic masks conditioned on a given background and bounding box location. 
% Our assumption is two folds, 1) The bounding box location substantially reduces the set of possible generated masks, 2) the background scene also reduces the set of possible masks, as it defines how the generated object should interact with its environment.
% We assume that combining these two inputs with a latent vector $\z_m \sim \mathcal{N}(0,\,1)$ can sample multiple realistic shapes and poses given annotated masks from a given object class. \ow{not sure we really need this paragraph} \jt{I also don't know what the point is.}

%\paragraph{Discussion:}
% each with varying object pose, object count, background, \etc~sampled from the respective domains $\S$ and $\T$. 
% Further, assume that each source image $\s \in \S$ is provided with an object segmentation mask $\s_{\m}\in\S_{\m}$. 
% Our goal is to learn a transfer function $f:\S\times\S_{\m}\to \T$ which translates objects in a source image $\s$ into objects in the target domain $\T$ in an output image $\mathbf{t}':=f(\s,\s_{\m})$.
% % We begin with source and target domains $\S,\T$ sampled as databases $S$ and $T$ of images of two object classes, each with varying object pose, object number, background, and so on. Given an image paired with its object segmentation mask $(\s, \s_{\m})$, our goal is to approximate a function $f$ such that $f(\s, \s_{\m}) = \mathbf{t}' \in \T$. 
% Figure \ref{fig:architecture} (left) visualizes our approach, as it relates to InstaGAN~\cite{instagan} (middle).

% %We may obtain $\mathbf{t}'$ using an auto-encoder; however, we wish to incorporate information from the segmentation mask in the decoding process. 
% As in InstaGAN~\cite{instagan}, we encode both $\s$ and $\s_{\m}$: $h_{\s} = \mathrm{enc}_\S(\s)$ and $h_{\s_{m}} = \mathrm{enc}_{\S_\M}(\s_{\m})$. Then, we concatenate these feature representations channel-wise and feed them: 1) into a decoder $\mathrm{dec}_\T$ which gives us $\mathbf{\hat{t}}'$, and 2) into a mask decoder $\mathrm{dec}_{\T_\M}$ which gives us $\mathbf{t}'_{\m}$.
% Formally this is expressed via $\mathbf{\hat{t}}' = G_\S(h_{\s}, h_{\s_{\m}})$, and $\mathbf{t}'_{\m}= G_{\S_\M}(h_{\s}, h_{\m_{\s}})$. Finally we obtain $\mathbf{t}'$ by feeding $\mathbf{\hat{t}}'$ to our differentiable blending module: $\mathbf{t}' = \text{Poissonblend}(\mathbf{\s, \hat{t}}', \s_{\m}, \mathbf{t}'_{\m})$. \ow{still refers to B} \ym{It is the same as the diagram now}

% To constrain our final results to look realistic, we use an adversarial discriminator $\D_\S$ which distinguishes between real pairs $(\s, \s_{\m})$ and fake pairs $(\mathbf{s}', \s'_m)$, where $\s'$ is the generated image from $\mathbf{t}\in\T$ (likewise for $\s'_{\m}$).
% The RGB and mask inputs are fed to the discriminator by first separately encoding them: $d_{\s} = \mathrm{enc}_{D_\S}(\s)$ and $d_{\s_{\m}} = \mathrm{enc}_{D_{\S_\M}}(\s_{\m})$. Then, similar to the generation part, we concatenate these feature representations channel-wise and feed them into a discriminator:
% $D_\S(d_{\s}, d_{\s_{\m}})$ gives us the probability of the pair $(\s, \s_{m})$ being real.


% In sum, we train an separate encoders for $\S$, $\S_\M$, $\T$, $\T_\M$, separate decoders for $\S$, $\S_\M$, $\T$, $\T_\M$, and separate discriminator encoders for $\D_\S$, $\D_{\S_\M}$, $\D_\T$, $\D_{\T_\M}$. 
% Their parameters are updated by playing the mini-max game governed by the Least Square GAN loss: 
% \begin{align}
%     \calL_\text{\emph{GAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) =& (D_\S(d_{\s}, d_{\s_{\m}}) -1)^2 +  \nonumber \\
%     &  (D_\T(d_{\mathbf{t}}, d_{\mathbf{t}_{\m}}) -1)^2 + \nonumber \\
%     & D_\S(d_{\mathbf{t}'}, d_{\mathbf{t}'_{m}})^2 + D_\T(d_{\s'}, d_{\s'_{m}})^2,
%     \label{eq:LSGAN}
% \end{align}
% where $\Theta_{D}$ contains the parameters of $D_\S, D_\T, D_{\S_\M}, D_{\T_\M}$, and $\Theta_{S}$ and $\Theta_{T}$ contain parameters of the encoding and decoding parts in $\S$, $\S_\M$ and $\T$, $\T_\M$ respectively.

%The system is joined cyclically such that all components involved in translations are trained simultaneously (Figure~\ref{fig:architecture}). Please see our supplemental material for details on the encoder and decoder architectures.


% \paragraph{Identity loss.}
% We also find that assisting the GAN objective with an identity loss, is necessary for convergence. Such loss  encourages the generated images to be identical to the inputs in the case where source and target domains are the same: \ym{Do we do that for both the mask and RGB or only RGB?}
% \begin{align}
%     \calL_{idt}(\Theta_{S}, \Theta_{T}) = \calL_{id}(\Theta_{S}, \Theta_{T}) + \calL_{id_{\m}}(\Theta_{S}, \Theta_{T}), 
% \end{align}
% such that:
% \begin{align}
%     \calL_{id}(\Theta_{S}, \Theta_{T}) =& \|\s -  G_\T(h_{\s}, h_{\s_{\m}})\|_1 + \nonumber \\  
%     &\|\mathbf{t} -  G_\S(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1, \nonumber\\
%     \calL_{id_{\m}}(\Theta_{S}, \Theta_{T}) =& \|\s_{\m} -  G_{\T_\M}(h_{\s}, h_{\s_{\m}})\|_1 + \nonumber \\
%     & \|\mathbf{t}_{\m} -  G_{\S_\M}(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1. \nonumber
% \end{align}

% Our final objective is hence written as: 
% \begin{align}
%     \calL(\Theta_{D}, \Theta_{S}, \Theta_{T}) = \calL_\text{\emph{GAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) + \lambda \calL_{idt}(\Theta_{S}, \Theta_{T}),
% \end{align}
% where $\lambda$ is a hyper-parameter that we fix to 10 \ym{check this}.

%We take lessons from InstaGAN’s use of segmentations and note that we can extend their use even further. 
%The segmentation masks provides us with not only the shape of the object but also its location. 
% We take advantage of the fact that the segmentations already define the areas of the image which need to be changed. Thus, we simply task our generator with creating a new foreground by “giving it” the background. We accomplish this by using a differentiable Poisson blend to restrict the output of our generator to the portion of it that lies within the. We slightly dilate the mask used to blend to allow our image generator how to modify areas around the foreground to make the blending more seamless.

% \paragraph{Poisson Blending Module}
% \ow{This part should be integrated into the above section. Instead of describing 1. instagan setup, then 2. our modifications, let's define 1. our architecture, and make sure we mention the similarity to instagan (and the differneces (missing loss fns)}
%Our Poisson module tasks the generator only to produce a new foreground while discarding the background. 
%Such behavior is possible by blending the newly generated foreground with the input background using the differentiable poisson blending algorithm described below. 
% From the discriminator point of view, it receives a generated image with a realistic background and a generated foreground. This encourages the generator to perfect its foreground generation in order for the mini-max game to converge.

% We build upon Farbman et al.'s convolution pyramid~\cite{farbman2011convolution} approximation of Poisson Blending~\cite{perez2003poisson}.
% The goal of this work is to reconstruct the image from its gradient field, where in Poisson Blending, the gradient field is composed of the foreground gradient composited onto the background gradient in the hole region.
% Poisson Blending involves finding a smooth ``membrane'' that interpolate of boundary colors on the hole by solving the Laplace equation. 
% This is computationally expensive, and convolution pyramids approximate it with an approximation of Shepard's ~\cite{shepard1968two} data interpolation method. 
%Shepard's
%Given a binary mask $\mathbf{m}$, a source image $\mathbf{s}$ and a target image $\mathbf{t}$, we first compute the mask boundary $\mathbf{b}$ by convolving $\mathbf{m}$ with a filter of size $3\times3$: $\mathbf{l} = [[0,-1,0],[-1,4,-1],[0,-1,0]]$. 
%Such filter, when convoluted on a region containing the same values, returns 0. Hence, when applied on the binary mask, $b=\mathbf{m}*\mathbf{l}$, only the boundary region will have non zero values. 
% \ow{I think we should actually put as little info as possible, as it is not our contribution, but that of convolution pyramids. I commented out the following section, but please check to see if you agree} \ym{Sounds good, I have put the maximum info possible as we can always truncate.}
%Shepard uses $\mathbf{b}$ to alter the source image via $\mathbf{s}'  =  \mathbf{s} + \mathbf{d}$, and $\mathbf{d}$ can be efficiently computed via: 
% \begin{align}
%     \mathbf{d}(x_i) = \frac{\sum_{j=0}^n d(x_i, x_j)\hat{b}(x_j)}{\sum_{j=0}^n d(x_i, x_j){b}(x_j)},
%     \label{eq:Shepard's}
% \end{align}
% where $d$ is a function that is inversely proportional to the distance between its inputs, $\hat b = b.(\mathbf{t} - \mathbf{s})$, and $n$ is the number of elements inside the mask. Note that, if $x_i$ is far away from the boundary then $d(x_i, x_j)$ will be close to zero. Meaning that $\mathbf{d}$ contains mostly zeros apart from the membrane surrounding the mask boundary, 
% which will contain values correcting the distribution shift in the source image compared to the target one. 

% Eq.~\ref{eq:Shepard's} is however not the most efficient, especially in our scenario where we are interested in reducing the computational cost of Image-to-Image translation. As such, Eq.~\ref{eq:Shepard's} can be seen as a ratio of convolutions that we approximate using convolutional pyramids~\cite{farbman2011convolution}. 

% Given an input $b$, we construct the convolutional pyramid output by first choosing the number of levels $L$ in the pyramid, then we feed the input to $L$ consecutive strided convolutions with a fixed kernel $h_1$, which performs the convolution operations while reducing the resolution of the input by half, formally this is expressed via: $b^{l+1} = \text{conv}(b^l, h_1)$, where the convolution here is computed using a stride of 2. 
% Then we compute the up-sampling pass by: $\hat b^{l} = \text{deconv}(\hat b^{l+1}, h_2) + \text{conv}(g, b^l)$, where $h_2$ and $g$ are both fixed kernels, with $\hat b^{L+1} = 0$. 
% The fixed kernels $h_1$, $h_2$ and $g$ are obtained by minimizing the $L_2$ norm between the output of the convolution pyramid and the desired linear transformation we wish to approximate, in our case Eq.~\ref{eq:Shepard's}. 
% Note that as a result of the numerical optimization, the kernels obtained are generalizable. In other terms they can be used on new images that have not been seen on the training set.

% By using such approach we can approximate the denominator and nominator of Eq.~\ref{eq:Shepard's} in linear time with respect to $n$, making our mappings from source to target and inversely run with minimal computations added compared to the vanilla GAN algorithm. 
% Most importantly, the convolutional pyramid used is fully differentiable which makes backpropagating through our network possible, This allows us to train with classical gradient based optimizers such as ADAM.

% The combination of real backgrounds and generated foregrounds as input to the discriminator is performed by blending the output of the generator to its input using as a mask the union of the real and generated foregrounds. The blending is an approximation of the well known Poisson blending using the previously discussed differentiable convolutional pyramids.


% \subsection{Simplified Objective Function}

% \vspace{.2cm}\noindent \textbf{Function.}

% \begin{align}
%     \calL_\text{\emph{GAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) =& (D_\S(d_{\s}, d_{\s_{\m}}) -1)^2 +  \nonumber \\
%     &  (D_\T(d_{\mathbf{t}}, d_{\mathbf{t}_{\m}}) -1)^2 + \nonumber \\
%     & D_\S(d_{\mathbf{t}'}, d_{\mathbf{t}'_{m}})^2 + D_\T(d_{\s'}, d_{\s'_{m}})^2,
%     \label{e:LSGAN}
% \end{align}
% where $\Theta_{D}$ contains the parameters of $D_\S, D_\T, D_{\S_\M}, D_{\T_\M}$, and $\Theta_{S}$ and $\Theta_{T}$ contain parameters of the encoding and decoding parts in $\S$, $\S_\M$ and $\T$, $\T_\M$ respectively.

% Note that compared to most of the image-to-image translation algorithms ~\cite{instagan, multimodal2018, almahairi2018augmented, yi2017dualgan}, our final loss function (Eq~\ref{eq:LSGAN}) is \emph{substantially} simplified, which allows our algorithm to train faster while focusing more on the GAN objective and hence, on the quality of generated images.
%Previous state of the art results have entailed cyclical loss functions~\cite{zhu2017unpaired}.
% While our training is entirely done by solely optimizing Eq.~\ref{eq:LSGAN}, the previous state of the art objectives~\cite{zhu2017unpaired,instagan}, are more complicated.
% Fig~\ref{fig:architecture} (middle) shows the InstaGAN architecture, consisting of the following loss functions:

% \begin{align}
%     \calL_\text{\emph{InstaGAN}}(\Theta_{D}, \Theta_{S},\Theta_{T}) =& \calL_\text{\emph{GAN}} + \lambda_1 * \calL_\text{\emph{idt}} +\nonumber\\
%     & \lambda_2 * \calL_\text{\emph{cycle}} + \lambda_3 * \calL_\text{\emph{ctx}},\nonumber
% \end{align}
% Where $\calL_\text{\emph{idt}}$ is an identity loss encouraging a generated images to be identical to itself in the case where source and target domains are the same:  

% \begin{align}
%     \calL_{idt}(\Theta_{S},\Theta_{T}) = \calL_{id}(\Theta_{S},\Theta_{T}) + \calL_{id_{\m}}(\Theta_{S},\Theta_{T}),\nonumber
% \end{align}
% with: 
% \begin{align}
%     \calL_{id}(\Theta_{S},\Theta_{T}) =& \|\s -  G_\T(h_{\s}, h_{\s_{\m}})\|_1 + \nonumber\\
%     &\|\mathbf{t} -  G_\S(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1, \nonumber
% \end{align}
% \begin{align}
%     \calL_{id_{\m}}(\Theta_{S},\Theta_{T}) =& \|\s_{\m} -  G_{\T_\M}(h_{\s}, h_{\s_{\m}})\|_1 + \\ &\|\mathbf{t}_{\m} -  G_{\S_\M}(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1.
% \end{align}
% and $\calL_{id_{\m}}$ serves the same purpose as $\calL_{id}(\Theta_{S},\Theta_{T})$ but applied on masks instead.

% Constraining the generation even further, the cyclic loss ensures that images are mapped to themselves when mapped from source to target and back to to source:  
% \begin{align}
%     &\calL_{cyclic}(\Theta_{S}, \Theta_{T}) = \calL_{cyc}(\Theta_{S},\Theta_{T}) +\calL_{cyc_{\m}}(\Theta_{S},\Theta_{T}), \nonumber\\
%     &\calL_{cyc}(\Theta_{S}, \Theta_{T}) = \| \s - \s''\|_1 + \| \mathbf{t} - \mathbf{t}''\|_1, \nonumber \\
%     &\calL_{cyc_{\m}}(\Theta_{S}, \Theta_{T}) = \| \s_{\m} - \s_{\m}''\|_1 + \| \mathbf{t}_{\m} - \mathbf{t}_{\m}''\|_1,\nonumber
% \end{align}
% where $\s'' = G_\T(h_{\s'}, h_{\s_{\m}'})$, with $h_{\s'} = E_\T(\s')$ and $h_{\s_{\m}'} = E_{\T_\M}(\s_{\m}')$. Likewise for $\s_{\m}''$.

% Finally, the \emph{context loss} enforces the \emph{intersection} of backgrounds in $\s_{\m}$ and $\mathbf{t}_{\m}'$ to not change: 
% \begin{align}
% \calL_{ctx}(\Theta_{S}, \Theta_{T}) =& \|(\s-\mathbf{t}') \odot w(\s_{\m}, \mathbf{t}_{\m}')\|_1  \nonumber + \\
% &\|(\mathbf{t}-\s') \odot w(\mathbf{t}_{\m}, \mathbf{s}_{m}')\|_1,
% \label{eq:ctx}
% \end{align}
% where $\odot$ represents Hadamard product and $w(\s_{\m}, \mathbf{t}_{\m}') =  1 - \max(\s_{\m}, \mathbf{t}_{\m}')$ . However since Eq.~\ref{eq:ctx} operates as a soft constraint, background changes and artifacts still occur as depicted in Fig.~\ref{tab:background_examples}.

% Removing the cycle consistency loss and the identity loss considerably decreases the computational overhead required to complete a forward pass, and emoving the context loss encourages the generator to focus only on the foreground generation.
% Using our differentiable blending module, we are left only the adversarial loss, similar to the original GAN proposed by Goodfellow et. al~\cite{goodfellow2014generative}.
% This has the added benefit of requiring fewer hyper-parameters to balance the different loss terms. 

%3) adding our differentiable blending module which simplifies the image-translation problem, enabling us to remove the previously discussed losses while improving the image quality.  

%\subsection{Advantages: Less is More}
% Our advantages over InstaGAN are threefold. Our approach: 
% \ag{Should this be 4?}
% \ms{Do you mean 4 contributions?}
% \begin{enumerate}
%     \item Halves the number of parameter updates required at each step of training through the removal of cyclic loss.
%     \item Removes the need for tuning hyperparameters for identity loss, cyclic loss and context loss.
%     \item Prevents the generator from:
%         \begin{enumerate}
%             \item reconstructing the background leading to compounding reconstruction error potential degradation of image quality.
%             \item reconstructing visual details that are lost during the translation. The generator no longer needs to wastefully steganographically encode this information~\cite{chu2017cyclesteg}. 
%         \end{enumerate}
% \end{enumerate}

%Our network does not require dataset specific tuning of these hyper parameters and is able to prevent background leakage with additional degrees of robustness. This simplicity makes our approach much more applicable to novice AI practitioners who may lack the domain knowledge and additional compute to train these models. 
% \ow{we need to show 1. the full loss function, and then 2. our reduced one, with clearly fewer terms.}

%We are able to abstract ourselves from InstaGANs losses and hence their hyperparameters by presenting the discriminator with images containing a generated foreground combined with a real background. This, in turn, encourages the generator to perfect its foreground generation and makes the image translation problem much simpler. Indeed, the generator's capacity is in this case not wasted on altering the background as an attempt to fool the discriminator but is solely devoted to generating a plausible foreground.  


% \paragraph{Sequential training:} As we are using object-centered datasets with mutilple instances, we use the same sequential training strategy as InstaGan. Given an image containing $n$ instances, we select their $n$ corresponding masks, then on each sequence iteration we feed the image and two masks to the generator until the $n$ masks are consumed. At the end of each iteration, we update the subsequent real image with the newly blended fake image.  If $n$ is odd, then we feed an empty mask alongside the final mask. 
% Fig~\ref{fig:architecture} (right), shows the sequential training strategy.
% The combination of real backgrounds and generated foregrounds as input to the discriminator is performed by blending the output of the generator to its input using as a mask the union of the real and generated foregrounds. The blending is an approximation of the well known poisson blending using the previously discussed differentiable convolutional pyramids.
% We wish to emphasize that our network architecture makes our generator mapping more restricted than other architectures. Our segmentation generator’s output is fed directly to the discriminator, so the regularization effects of the discriminator restrict the generator’s segmentations to realistic objects in the target domain. If the generator were to create abstract segmentations, it would be penalized.

% Since, our image generator may only modify areas within this segmentation, it does not attempt some of the strategies taken by generators of other architectures, such as contorting the background or changing the image’s lighting. Thus, we are able to remove the identity and cylic losses. 

% Our discriminators are also multi-scale, which has demonstrated better results on these tasks~\cite{Gokaslan2018, multimodal2018,Li2018UnsupervisedIT}.

% \paragraph{Cyclic loss.}
% Unpaired image translation is an under-constrained problem even with $\calL_\text{\emph{GAN}}$.
% To further constrain it, we adopt the Zhu et al.~\cite{zhu2017unpaired} cyclic consistency which helps conserve characteristics of the input image (\eg, the pose of the object).
% For this purpose, we could use a cycle energy loss on both the input images and their masks. This encourages an image mapped twice (from source to target to source) to be identical to the original image:
% \begin{align}
%     \calL_{cyc}(\Theta_{S}, \Theta_{T}) &= \| \s - \s''\|_1 + \| \mathbf{t} - \mathbf{t}''\|_1, \\
%     \calL_{cyc_{\m}}(\Theta_{S}, \Theta_{T}) &= \| \s_{\m} - \s_{\m}''\|_1 + \| \mathbf{t}_{\m} - \mathbf{t}_{\m}''\|_1,
% \end{align}
% where $\s'' = G_\T(h_{\s'}, h_{\s_{\m}'})$, with $h_{\s'} = E_\T(\s')$ and $h_{\s_{\m}'} = E_{\T_\M}(\s_{\m}')$. Likewise for $\s_{\m}''$. %\kimki{I guess the squared terms in the above equations are mistakes?}\ym{which squared terms? we followed the InstaGAN setting where the cycle energies are not squared.}\kimki{I mean, having the norm squared in the source domain terms but not in the target domain terms??} \ym{yup sorry you are right} \kimki{Thanks}

% While cyclic loss both aids the network in preventing mode collapse and in preserving attributes across domains, the term has limitations. The bijective constraint can hinder shape change~\cite{Gokaslan2018, zhu2017unpaired} and texture transfer. Small irrelevant details must be preserved to perfectly reconstruct the original image. Instead, we focus on reconstructing a much simpler task: the original segmentation. In our results, we will show empirically that minimizing only $ \calL_{cyc_{\m}}$ is enough to achieve the goal initially desired by cycle energies.

% We find that eliminating the RGB reconstruction loss improves the quality of generated images (Table~\ref{t:kid_ablation}). The remaining loss terms provide adequate stability to the network to prevent mode collapse. Furthermore, unlike previous methods which do not require cyclic reconstruction~\cite{benaim2017one}, our method can handle shape change.

%\begin{align}
%    \calL_{id} =& \|\s -  G_\T(h_{\s}, h_{\s_{\m}})\|_1 +  \nonumber \\ 
%    &\|\mathbf{t} -  G_\S(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1,
%\end{align}
%\begin{align}
%    \calL_{id_{\m}} =& \|\s_{\m} -  G_{\T_\M}(h_{\s}, h_{\s_{\m}})\|_1 +  \nonumber \\
%     &\|\mathbf{t}_{\m} -  G_{\S_\M}(h_{\mathbf{t}}, h_{\mathbf{t}_{\m}})\|_1.
%\end{align}
% \paragraph{Context loss.}
% Jointly optimizing the previous three losses enables shape change for image-to-image translation; however, there is no mechanism encouraging only foreground objects of interest to be altered, \eg, in the giraffe to sheep problem, one should be able to change a giraffe to the corresponding sheep without altering the background.
% One way to achieve such property is to enforce the initial background pixels in $\s$ and given by $\s_{\m}$ not to change in $\mathbf{t}'$.
% However, doing so would be in opposition with our initial motivation of performing significant shape changes across domains as, in that scenario, pixels which were initially in the background of $\s$ could end up being in the foreground of $\mathbf{t}'$.
% For this reason, we instead enforce the \emph{intersection} of backgrounds in $\s_{\m}$ and $\mathbf{t}_{\m}'$ not to change, which allows for shape change while encouraging the background to be conserved as in InstaGAN
% % \kimki{Can we remove `That is:' and finish the previous sentence as `to be conserved:'?} That is: %\jt{edited equations back}
% \begin{align}
% \calL_{ctx}(\Theta_{S}, \Theta_{T}) =& \|(\s-\mathbf{t}') \odot w(\s_{\m}, \mathbf{t}_{\m}')\|_1  \nonumber + \\
% &\|(\mathbf{t}-\s') \odot w(\mathbf{t}_{\m}, \mathbf{s}_{m}')\|_1,
% \end{align}
% where $\odot$ represents Hadamard product and $w(\s_{\m}, \mathbf{t}_{\m}') =  1 - \max(\tilde{\s}_{\m}, \tilde{\mathbf{t}}_{\m}')$ with $\tilde{\s}_{\m}$ being the binary, rounded version of the initial mask. Furthermore, since this constraint operates as a soft constraint, the network may make small changes outside the segmentation that enhance the plausibility of the image. For instance, filling gaps in between segmentation or slightly changing the lighting tone or vegetation in an image.

% \paragraph{Feature matching loss.} Finally, we define a feature matching loss which we find to encourage sharper and more realistic images. This loss encourages feature representations computed from $\{\mathbf{s}'_i\}_{i=1}^{N_t}$ to be close in terms of the $L2$ norm with respect to the features computed from $\{\mathbf{s}_i\}_{i=1}^{N_s}$, where $N_s$ and $N_t$ are the number of datapoints for domains $\S$ and $\T$ respectively. 
% %\kimki{Can we use the term L2 distance instead of Euclidean distance as we already used $\|\cdot\|_2$?}\kimki{What is $N$? The number of images? Can an image have multiple objects?}\ym{addressed}\ag{Can we fix the double subscript Latex issue?}\ym{which one, I thought this was solved as I dropped the i indices?} 
% Such feature representations are extracted in this case from $D_\S$. 

% This loss has been shown to help produce good generated images~\cite{salimans2016improved,wang2017pix2pixHD,Gokaslan2018,wang2018vid2vid}. The intuitive reason why this works is that we wish neurons in the source domain discriminator to be activated in the same way between generated source images and real ones. This ends up reinforcing the realism of the generator, $G_\S$ in this case.

% Formally, we express this via the following loss: 
% \begin{align}
%     \calL_{FM}(\Theta_{S}, \Theta_{T}) = \sum_{l=1}^{L-1} &\E_{\s \sim B}(\|D_\S^l(\s') - D_\S^l(\mathbf{s})\|_2^2) + \nonumber \\ 
%     &\E_{\mathbf{t} \sim B}(\|D_\T^l(\mathbf{t}') - D_\T^l(\mathbf{t})\|_2^2), \label{eq:FM}
% \end{align}
% %\kimki{A quick question: the expectations above are just sums over data points within the mini-batch $B$. Is it correct?}\ym{Indeed}\kimki{Thanks. Summation might be easier to understand than this mathematically ill-defined expectation symbol in this case. But this notation is well-established :(.}
% where $L$ is the number of layers in the discriminator architecture, $B$ is the mini-batch, and $D^l$ is the feature activation of the corresponding discriminator at layer $l$. Moreover, since we use a small batch size, directly enforcing Eq.~\ref{eq:FM} %
% %Eq.~\eqref{eq:FM} 
% may be less valid for a given pair of $s_i'$ and $s_i$. We introduce the novel contribution of maintaining an exponential moving average for feature representations of the real images and use them instead in Eq.~\ref{eq:FM}. 

 

% \paragraph{InstaGAN3D:}
%  this model builds upon InstaGAN and improves it by adding two adversaries, the first discriminates between real and generated segmentation masks, while the second discriminates between real and generated images.  
%  Trained jointly with the initial discriminator, we find that doing so encourages sharper generated images, see Figure.


% Our work is inspired by recent works such as ContrastGAN~\cite{liang2017} and InstaGAN~\cite{instagan} which augment CycleGAN with a segmentation map. We make several important changes, each of which meaningfully improves the translation quality as we show in the ablation study (Sec.~\ref{s:results}). For clarity, we list all changes below.

% \vspace{.2cm}\noindent \textbf{Additions.}
% Over losses in InstaGAN, we add relativistic average discriminators~\cite{jolicoeurRelativistic} via least squares GAN~\cite{mao2017least}, multi-scale discriminators, and feature matching loss. We also maintain an exponential moving average over the feature match loss to learn the feature statistics of real images across the entire dataset despite the small minibatch size.

% \vspace{.2cm}\noindent \textbf{Subtractions.}
% We remove the `\emph{insta}nce' from InstaGAN: We only provide one mask per image which contains the intersection of all per-instance masks, instead of one mask per instance in the image framed as recursive segmentation. This reduces complexity and avoids the need for expensive explicit instance segmentation. We show that this still achieves high quality results. Further, we do not enforce a cyclic loss on the RGB reconstruction and only on the mask reconstruction, which again saves computation.



%minimizing the cycle loss energy with respect to real and generated images can prevent shape change as CycleGAN~\cite{zhu2017unpaired} demonstrates. 
%InstaGAN manages to counter this effect by using additional supervision, however minimizing the cycle energy in that way, forces the generator to smartly hide source domain information (e.g. the neck of a Giraffe) by partly in-painting them (See Figure\ref{}), which produces artifacts on the final result.
%We reduce this effect by enforcing a weaker cycle energy that only acts on the masks (i.e we only reconstruct the masks). Doing so, removes the burden of reconstructing textures while encourages properties such as the pose to be conserved.



==> src/4-experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\import{\figDirCVPR}{fig_giraffe_zebra}
\import{\figDirCVPR}{fig_pizza}

\paragraph{Datasets:} 
%We train our algorithm on classes from COCO~\cite{MSCOCO2014} which contains challenging images with many object appearances, poses, perspectives, possibly occluded, and with some noisy annotations.
We extract three classes from COCO: \emph{Giraffe} (2,205 images), \emph{Zebra} (2,306 images), \emph{Pizza} (2,623 images).
The first two classes have high shape variation, while the last one contains a high texture variation. 
We exclude all instances which are smaller than 1\% of the entire image, all masks containing multiple separate components and the ones that intersect with the image borders.
Background images for stamping are collected from the Internet by searching relevant queries under a `free to use and modify' license, and will be released alongside our code.

\vspace{-0.25cm}
\paragraph{Training:} We train our shape generation network for 1000 epochs on all datasets, and our texture network for 400 epochs. We use a batch size of 4 and train all our models on 4 GPUs (NVIDIA GTX 1080 Ti).
We use instance normalization in all hidden layers of both generators. 
We use the ADAM optimizer with a learning rate of 0.0002, $\beta_1 = 0.5$ and $\beta_2 = 0.99$. 
We decrease the learning rate linearly towards 0 at half training.
In our loss, all $\lambda$ hyperparameters are fixed to 10 apart from $\lambda_{KL}^T$ which is set to 0.05.
We set random vectors sizes to $|\z_m|=128$ and $|\z_i|= |\z'_i| =8$. 

% We fix the hyperparameters $\lambda_i$ to 10. \ow{move this to where $\lambda$ is described?}
% We fix $\lambda_{1-5}$ to 10 and $\lambda_6$ to 0 apart for the giraffe dataset where it is set to 10.

%\vspace{-0.1cm}
\subsection{Method comparisons}
%We compare our algorithm with two state of the art composition-based image generation algorithms.
We are not aware of any methods that addresses our exact problem, and so we adapt close-by methods for comparison.
%our approach and describe the modifications necessary for comparison.


\vspace{-0.25cm}
\paragraph{Semantic image manipulation of Hong et al.~\cite{HierarchicalSemanticImageManpulation}:}
This approach uses multi-class pixel-wise segmentation maps to exploit scene context, from which we extract per-class binary masks.
In this setting, their method produces less distinct shapes and blurrier textures than our approach (Fig.~\ref{fig:giraffezebra}).  
Further, Hong et al.'s algorithm is deterministic: it insert only one instance given a bounding box, whereas our approach can create multiple shapes and textures from the same bounding box.
Finally, Hong et al.~generate content for the entire bounding box, which requires solving the more difficult task of also generating background regions which match seamlessly with the rest of the content (Fig.~\ref{fig:pizza}).


\vspace{-0.25cm}
\paragraph{FineGAN~\cite{finegan}:} This whole-image approach decomposes generation into first generating the background and then the foreground. 
It produces convincing results on low variance datasets such as bird images of CUB~\cite{WelinderEtal2010}. 
However, when trained on our classes from COCO, performance tend to decrease (Figs.~\ref{fig:giraffezebra} \& \ref{fig:pizza}), or collapse altogether.
Further, while FineGAN allows for stochastic texture generation, it cannot generate localized instances for user control over the scene layout, \eg, generated foregrounds are often in the center of the image. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Forward declaration
\import{\tableDir}{KID_texture}
\import{\tableDir}{KID_masks}
\import{\tableDir}{KID_compare}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\jt{Also maybe a `what happens when you put the object in the sky?' type figure.}
\import{\figDirCVPR}{instanceReplacement}
\import{\figDirCVPR}{instanceInsertion}


\vspace{-0.25cm}
\paragraph{Copy and Paste + Deep Harmonization~\cite{tsaiCVPR2017}:}  
We also compare with a copy and paste baseline, where we look in the training set for masks that most resembles the ones our algorithm generates.
Rather than a simple nearest neighbor search, we crop each training mask and re-scale it to fit the size of our generated ones. Then, we compute the corresponding cosine distance which computes the angle between its inputs and is usually used for binary data. The training mask with the smallest score is selected. 
% \ow{what does this do? affine invariant nearest neighbor?}\ym{added this, but not sure it helps}
Moreover, to make this baseline even more realistic, we use a state of the art harmonization approach~\cite{tsaiCVPR2017}. 
Results are shown in Figures \ref{fig:giraffezebra} and \ref{fig:pizza}, from where we can see that that this baseline often struggles to form a convincing composite. 
Furthermore, this approach has several other limitations: without using our model's generated mask to query the database, the user would be required to provide an actual mask rather than a bounding box. 
In addition, it requires a substantial amount of time to search through the training dataset, and is not able to disentangle shape from texture.



\subsection{Additional Applications} 

Beyond \emph{object stamps}, our algorithm can \emph{retexture} an existing object instance in an image (Fig.~\ref{fig:instanceReplacement}).
With these `ground truth' masks, our algorithm generates realistic textures that blend correctly with their respective backgrounds, \eg, the sides of the generated pizzas contain doughy edges, as real pizza has.
Alternately, our method supports applications where a user would like to insert an object of a specific shape into a given background, and have it be textured realistically (Fig~\ref{fig:instanceInsertion}). %Here, we 
%Our algorithm allows him to do so by using $G_T$. 
%application, where masks from the validation set are used.in the case where the user 


\subsection{Quantitative Evaluation}

We use KID~\cite{bisuargr18} as an evaluation metric as it has been shown to give more consistent results than Frechet Inception Distance (FID), especially with small numbers of generated samples~\cite{heusel2017gans}.

\vspace{-0.25cm}
\paragraph{Semantic image manipulation of Hong et al.~\cite{HierarchicalSemanticImageManpulation}:} As this approach is deterministic, we generate one instance per bounding box and per scene. We do the same for our method using the same bounding boxes and background images. We report KID results on 50 random subsamples in table~\ref{tab:KIDcompare}. Our approach consistently performs better which agrees with the visual results (Fig.~\ref{fig:giraffezebra}). 

\vspace{-0.25cm}
\paragraph{FineGAN~\cite{finegan}:} We trained FineGan on the coco classes using a higher resolution than used in their paper, but equal to the one we use (256x256). On this setting FineGan has collapsed. As such, we used their original resolution (128x128) and bilinearly upsample the generated images to 256x256. 

FineGan is a whole image generation approach, and so a comparison using our composited foregrounds would not be fair. Instead, we compute KID using only generated foregrounds without compositing them with the backgrounds.
Table~\ref{tab:KIDcompare} shows the corresponding scores. FineGAN have substantially higher KID scores compared to us. This is due to many factors. FineGan is designed for datasets containing a hierarchical structure, for example `birds' whcih contain multiple species and shapes. Running the algorithm on classes such as `giraffe' and `zebra' results on a significant drop in diversity as shown in figure~\ref{fig:giraffezebra}. Moreover, resizing the images to 256x256 introduces artifacts that are captured by KID. 
% \emph{Note:} FineGAN collapses when trained on our higher resolution imagery (256x256), and so we bilinearly upsample their results from the resolution used in their paper (128x128).

\vspace{-0.25cm}
\paragraph{Ablation studies:}

We conduct a number of ablation studies. 
First, we evaluate which components of our method contribute to the quality of texture generation (Tab~\ref{tab:KIDtexture}). 
In this test, we generate a set of synthesized foregrounds by creating 10 different textures per instance mask in the validation set.
We then create 50 random subsets of real and generated images, and compute KID scores on them.
This evaluate is done on the `pizza' class due to the high texture variety. 
Our full method performs best, where removing the noise input (Noise) makes a small difference, removing the feature matching loss (FM, Eq.~\ref{eq:Loss_T_FM}) contributes to a larger degree.
Removing the bicycle loss (Bicycle) yields realistic results, but without diversity, which accounts for the higher KID score, and removing the VGG feature loss has the largest impact on result quality. 

We similarly ablate our mask generation, in this case on the `giraffe' class due to the high shape variation; we generate ten masks per bounding box in the validation set, then we construct 50 subsets to use for KID computation. Results are displayed in Table~\ref{tab:KIDmask}.

First, we remove the contribution of the feature matching loss in Eq.~\ref{eq:Loss_M_FM} and notice a score increase indicating that the FM loss helps in this task. Second, we try to reconstruct $\z_m$ from the generated mask directly instead from the predicted ADAIN parameters. In this setting (`Ours-mrecon'), our generator ignores the latent vector $\z_m$ which kills the shape diversity hence increasing the KID values. 
Finally, we try conditioning the mask discriminator using $s$ on top of $\m$ and $\b$ (`Ours-bgcond') but we did not notice any significant improvement (also discussed in \cite{zhu2017bicycle, pathak2016context}).

The cause of the high standard deviations in tables~\ref{tab:KIDtexture},~\ref{tab:KIDmask} are due to the differences in the selected subsets themselves; 
In the second column of both tables, we show the percentage of time each approach achieves the best score out of the 50 sub-samples used to compute the KID scores (referred to as 'Count' on the tables). As such, the standard deviations in that sense are still meaningful. 
% \ym{We should say somewhere that we will add a failure case figure int eh supplemetnal}


% \ms{Should we also ablate the reconstruction loss as it is important for diversity? I remember we tried quite a few schemes before getting to BicycleGAN.}


% We train a network which predicts the foreground directly from the cropped background $i_c$ without the first step of predicting the object mask (Fig.~\ref{fig:ablation} Top). 
% We see artifacts on both the generated foregrounds and the real backgrounds. 
% Without masks, we need to threshold the foreground to composite it on the background, which creates artifacts such as holes when the generator has failed to produce a realistic result.
% In addition, results from this approach don't blend properly with the background. 
% We also ablate the removal of the object discriminator $D_O$ and its associated losses (Fig.~\ref{fig:ablation} Middle). 
% This approach again adds artifacts to the generated foregrounds. 
% In rare cases, our algorithm may also show these artifacts (Fig.~\ref{fig:ablation} Bottom);  %(Fig.~\ref{fig:failure} Middle); 
% however, removing $D_O$ makes them ever present.
%\ow{are we predicting masks as well as fg here? that would be the fair comparison right? it seounds like we predict FG and then derive a mask from that?}

%  in this scenario we are left with only two discriminators and hence the losses \kimki{$\calL_{D_O}$, $\calL_{G_I}^O$, and $\calL_{FM}$?} $\calL_{D_t}$, $\calL_{G_t}$ and $\calL_{FM}$ are also discarded. 

% \import{\figDir}{fig_ablation}

==> src/5-discussion-old.tex <==
\section{Discussion}

\kimki{We proposed an algorithm that significantly simplifies object composition task. Our algorithm receives a target background image and an object bounding box that dictates the location and the scale of the object to be placed, and realistically blends the synthesized objects into the background. }


generates foreground objects and places them in the target background based on the user-provided bounding boxes, significantly simplifying object composition tasks. Our  }


\jt{When we talk about `pose' and 'shape', really neither of these things is true. Maybe this is a discussion point - we don't know about the giraffe skeleton and only know raster masks.}

\jt{Comparison to the joint vs. curriculum learning method, i.e., a $G_{mf}$?}\kimki{Youssef tried: joint learning is worse but this network has not been saved. So, we cannot include the results in the paper.}

\kimki{Comparison to training $G_m$ first and then, given fixed $G_m$, to train $G_f$ (in contrast to method described in `Training but for real' section?)} \jt{If we tried it (ever), we can just say that it didn't work/major fails...?} \ym{This sounds familiar but I can't say for sure I have tried it.}

\kimki{We could add an `algorithm' table showing how the training is actually done based on the final loss $\calL()$, maybe in the supplemental.} 

\jt{Also maybe a `what happens when you put the object in the sky?' type figure.}

\paragraph{Limitations}


\paragraph{Conclusions}

In conclusion, we have presented a method that allows users to generate object stamps on background images. This 

% We posit that ground truth pixel-wise mask segmentations provide two critical pieces of information to the network: localization of the object(s) in the image, and disentanglement of the (textureless) shape characteristics of the object.
% Bounding boxes provide the location of objects but do not reveal any information about their shape. 
% Rectangles possess poor IOU with the ground truth segmentations of animals such as giraffes (Table~\ref{tab:jaccard}). 
% Further, the network becomes biased towards rectangular shapes (Table~\ref{}) \ym{Do we have visual examples of this property?}. 

% The lower result quality from bounding boxes demonstrate that the shape hints provided by richer segmentation are important.
% However, lower quality masks generated from Deep GrabCut on bounding boxes~\cite{xu2017DeepCut} still produce good results both quantitatively and qualitatively (Fig.~\ref{tab:Supervision1}). 
%\kimki{I wonder if we need to reduce the scope of `low-quality' masks a bit further: Bounding box annotations could also be considered low-quality and this doesn't work. Can we conclude that fine-grained supervision is better than box supervision even when they are erroneous?}

%\kimki{The discussion specifically in this paragraph seems to focus on how accurate or inaccurate supervision is rather than how weak or strong supervision is. I think in the rest of the paper, `weak' refers to a form of supervision, in accordance with commonly used term `weakly supervised learning' where the form of supervision varies (\eg from segmentation masks, to bounding boxes, and then to object centers; See slides 2: https://hbilen.github.io/wsl-cvpr18.github.io/assets/wsod.pdf)? I wonder if we should call this paragraph `... effectiveness of weak supervision' or instead, call it `... effectiveness inaccurate supervision'.}\jt{In masks? I don't think so.}\kimki{Resolved.}

% \paragraph{Full supervision cyclic failure.}
% In our supplemental, we demonstrate the bird to airplane dataset. 
% In this case, Deep GrabCut outperforms the fully supervised masks; even CycleGAN performs well.
% The human-provided segmentations hurt network performance both qualitatively and in terms of KID score. 
% We posit that this is because of images containing flocks of birds in the distance, which produce many small clustered mask regions which are hard to translate or reproduce cyclically.
% For these regions, that imprecise supervision is less specific is beneficial.

%\ow{TODO: finish this section, also this discussion is referenced earlier as well (Sec 4.1), it should occur in one place only}

%TODO MAybe fit in Peak Reponse Mapping 

%\import{\figDir}{masksupervision}
%\import{\figDir}{masksupervision_supplemental}
%\import{\figDir}{supervisionlevels}
%\import{\figDir}{supervisionlevels_supplemental}


% \paragraph{Object complexities.}
% Small objects in general can be difficult to segment effectively (both for human labelers and for automatic or semi-automatic methods). Localizing small and distant objects such as kitchenware and utensils in an unsupervised manner is difficult and requires at least some mask supervision. Furthermore, small objects that occur with common objects, such as bottles with humans, can also be unrecognized by cosegmentation approaches.

% Additionally, approaches can struggle even in the supervised case when two classes appear in the same image, \eg, a bus-to-car translation where images of buses often also contain a car. Therefore, the generator can learn the trivial solution which switches car and bus segmentation labels; this satisfies the bijective requirement by exploiting the RGB input to re-segment the object.

% \paragraph{Backgrounds.}
% Controlling background differences remains a challenging problem: the context loss constraint on background changes must be weighted with other losses, which allows the system some freedom. This can be desirable when modifying the background yields a more believable image, such as in changing content close to the mask to better cope with object shape changes. These cases tend to rely on the backgrounds already having at least some similarity, e.g., in animal conversions with natural landscape backgrounds. However, it can also yield poor results when backgrounds differ more. Our fire hydrant/toilet examples show generally higher KID scores as backgrounds from street scenes merge into bathrooms (Fig.~\ref{tab:Supervision1}, bottom). Increasing the context loss significantly can slow down or halt training as the discriminator becomes increasingly reliant on the background patches which the generator is unable to change. Future work may seek to find a better soft attention mechanism than concatenation.

% \subsection{Additional experiments}

% \paragraph{GrabCut.} We experimented with GrabCut~\cite{rother2004grabcut} vs.~Deep GrabCut, which presents a classic speed/performance trade-off. While less computationally expensive, GrabCut produced worse KID score in almost all cases compared to Deep GrabCut~\cite{xu2017DeepCut}, except for `elephant to bear'.

% \paragraph{Explicit foreground discriminator.} Inspired by ContrastGAN's strategy to only look at cropped patches within a discriminator, we introduce a variant with a separate second discriminator on only the predicted foreground region. This uses the RGB encoder of the domain's discriminator. We found that this approach \jt{....} \jt{This is InstaGAN2D?; but that's a bad name... Ours (+ explicit foreground discriminator}\ym{InstaGAN2D adds a discriminator on the masks. In this case a discriminator is added on the foreground RGB objects}

% \paragraph{Other approaches.}
% We also explored using the discriminator to localize the object and generate segmentations but found that the training process makes the network ill-suited for this task~\cite{kastaniotis2018attention}. \jt{I don't follow what we did here.}\kimki{I would suggest to remove this `Other approaches' paragraph as the observation made here is in line with related `Co-attention within the model' approaches. If not, can we move this paragraph to the end of this subsection, or rename it to something else than `Other approaches'?}

%Attention CycleGAN frameworks work well when little shape change is involved, but ultimately struggle when dealing with domains of differing shapes. 

% \paragraph{Explicit segmentation discriminator.}
% We also tried adding an additional discriminator which only looked at the segmentation channel. While it did improve mask quality, it did so at the expense of RGB quality. Furthermore, it performed worse with imprecise supervised masks and had a habit of adding additional instances of the animal.

% \paragraph{CycleGAN with mask concatenated.}
% Concatenating the segmentation masks to the RGB channels in CycleGAN led the network to produce all-black masks. By focusing only on the RGB channels, CycleGAN minimized the L1 cyclic loss. Since most of the background mask region is black, a trivial minimizer makes the entire mask image black.

% \paragraph{Unsupervised attention.}
% Using automatically-learned attention maps~\cite{mejjati2018unsupervised, chen2018attentiongan} turned out not to be robust to shape change. These algorithms constrain the generator to only modify attended regions in the image; however, if the source and target domains are not of the same shape, such an assumption can be constraining. For example, it is challenging to transform a sheep to a giraffe by only modifying pixels covered by the sheep. Consequently, these networks end up attending to the entire image to converge, which is similar to the CycleGAN setting.
% We tried training a coattention network from scratch along with the models, but we achieved poor shape change results. Ultimately, we found that transfer learned attention networks performed best while our end to end frameworks achieved poor results. The adversarial nature of training seems to often interfere with coattention.
% \ag{Youssef could you expand on this section?}\ym{done}

% \paragraph{Restricting the Images to Bounding Box}
% We also tried editing only the bounding box regions as is done in \cite{liang2017}. We found that doing actually negatively affected shape both KID and shape training results due issues with blending the image and the highly varying aspect ratio making the task more difficult. This approach may work on higher resolution images though.

%\section{Future Work}
% While we have shown that imprecise supervision can be helpful for challenging image-to-image translation tasks, more work is needed to enable robust shape change in a fully unsupervised manner (Fig.~\ref{tab:Supervision1}; CycleGAN struggles). Recent work has made strides enabling unsupervised shape change~\cite{Gokaslan2018}; however, they still alter the background significantly. Unsupervised attention-based approaches successfully conserve the background~\cite{mejjati2018unsupervised}, but can only deal with limited shape change. Future work should combine these properties to enable instance-aware image translation while simultaneously disentangling the background.
% % ensuring these work do not ensure \ym{this last sentence is weird (uses ensure two times.)} the consistency of the background. 

% Moreover, our approach is agnostic to the precision, type, and creation method of the segmentation masks. Future work may achieve higher performance by more closely integrating these differences into the model. We could also train on several classes at once as per other recent works ~\cite{almahairi2018augmented,choi2017stargan,multimodal2018,lee2018diverse,liang2017,royer2017xgan}.

% Recent work exists on learning segmentations using multiclass labels~\cite{kolesnikov2016seed,Zhou2018PRM}. Additionally, other recen

==> src/5-discussion.tex <==
\vspace{-0.25pt}
\section{Discussion}

Our method is one step in the direction of easy to use, high level control for guided image creation. 
However, this is a challenging problem, and there are still a number of limitations of this approach (see failure case figure in the supplemental material). 

First, we note that the COCO dataset is especially challenging, including issues from its instance annotations. 
For example, some instances are occluded, which causes holes in the masks. As such, sampling from the learned mask generator can create shapes with irregularities.
% (Fig.~\ref{fig:ablation} Bottom).  %(Fig.~\ref{fig:failure}). 
Some instances also only show parts of the objects, e.g., only the head of the giraffe, which can lead to some unexpected masks at test time.

Finally, with datasets containing complicated and diverse textures, texture generation can also be challenging; see the class \emph{Bus} in the supplemental material, where complex structured appearance with transparency through the windows is difficult to model.
% (Fig.~\ref{fig:ablation}).  %(Fig.~\ref{fig:failure}). 
%As generative models improve and are able to handle increased variance in datasets, we similarly expect that the quality of our approach will be greatly helped. 
For less complex classes, our approach allows users to sample the generator to obtain both object shapes and textures that they like. 

%\import{\figDir}{fig_failure}

\vspace{-0.25pt}
\section{Conclusion}

Inspired by curriculum learning, we have presented a method to generate object stamps by splitting the process into generating an object mask and object texture. Our approach carefully considers how to promote both detail and diverse generation in both shapes and texture, through feature match, perceptual, and auxiliary losses via conditioning vector encoder-decoders.
Further, we allow conditioning generation on background content. For this, we describe a way to train our approach on pre-existing segmentation datasets which \emph{include} object instances already but do not confuse the generator. Put together, this provides flexible generation across shape and texture via a simple bounding box interface.


==> src/6-relegatednotes.tex <==
% \section{Notes relegated to the back because James wanted a clean paper.}

% \subsection{Intro}

% \jt{Do any previous techniques actually propose to use bounding boxes, or bounding boxes with automatically-refined masks? This is itself a contribution if we can show somewhat similar performance.}
% \ag{I couldn't find any that did so. I did several papers that tried to extract masks from bounding boxes, but none the actually used the segmentations for anything after the fact.}

% \jt{New idea for supervision: paired `synthetic' data where we just change one object for another. Paste random giraffe and sheep cutouts (using gt masks) onto the same empty background image.}
% \ag{See learning to segment via cut and paste}

% \subsection{Method}

% \kimki{Here we define different functions as well as the corresponding training strategies (losses). We could define these functions earlier (\eg by providing a table) and here focus on the training methods?}

%\kimki{I hate when people use a reserved word like `relativistic' to represent something else : (.} \jt{what's another word for the operation? maybe we can change the lingo?}\kimki{Simply `relational' or `comparative'?}

==> src/X-segmentation.tex <==

% \section{Segmentation ideas}
% The goal is to have an algorithm similar to MUNIT/DRIT, however instead of encoding the `style' and `content' we wish to encode the `foreground' and `background'. The advantage of having such an algorithm is that given two images, it would be possible to swap their foregrounds which is similar (or at least a good step forward) to our final goal. 

% Given an image $x \in X$, with $X$ being an image domain formed by training data.  We wish to approximate (same applies for $Y$): 
% \begin{itemize}
%     \item Parameters of a attention autoencoder $A_X$ that takes the input image $x$ and outputs its mask $M_x$.
%     \item Parameters of a encoder $F_X$ that takes as input the foreground image $x \odot M_x$ and outputs its feature representation $f_x$.
%     \item Parameters of a encoder $B_X$ that takes as input the background image $x \odot (1-M_x)$ and outputs its feature representation $b_x$.
%     \item Parameters of a generator $G_X$ that is able to reconstruct the input image $x$ given its foreground and background representations $f_x$ and $b_x$.
%     \item Parameters of a discriminator $D_X$ that is trained to distinguish between real images from $X$ and generated ones. 
% \end{itemize}
% Note that in contrast with MUNIT/DRIT, this setting enforces that the inputs to $F_X$ and $B_X$ are from `opposite' domains induced by $M_x$ and $1-M_x$ respectively. Combined with the different constraints (given by energies to minimize bellow), this would eventually encourage $F_X$ to encode the foreground and $B_X$ to encode the background.

% Similar to MUNIT we wish to minimize several reconstruction energies: 

% \begin{align}
%     L_{recon_x} = \|x - \hat{x}\|_1,
% \end{align}
%  which is the standard reconstruction energy on the input image, with $\hat{x} = G_x(f_x, b_x)$.
% \begin{align}
%     L_{recon_{f_x}} = \|f_x - F_x(A_X(G_x(f_x, b_y)) \odot G_x(f_x, b_y))\|_1,
% \end{align}
%  with $A_X(G_x(f_x, b_y)) \odot G_x(f_x, b_y)$ being the estimated foreground of the generated image $G_x(f_x, b_y)$. 
% \begin{align}
%     L_{recon_{b_x}} = \|b_y - B_x( (1-A_X(G_x(f_x, b_y)))\odot G_x(f_x, b_y) )\|_1,
% \end{align}
% with $(1-A_X(G_x(f_x, b_y))) \odot G_x(f_x, b_y)$ being the estimated background of the generated image $G_x(f_x, b_y)$. 
% \begin{align}
%     L_{recon_{M_x}} = \|M_x - A_x(G_x(f_x, b_x))\|_1,
% \end{align}
%  which is a new reconstruction energy associated with the mask $M_x$.

% The mapping between domains $X$ and $Y$ is performed similarly to MUNIT, by switching the foreground vectors. For example a sample of the mapping $X \rightarrow Y$ is obtained via $\hat{y} = G_Y(f_y, b_x)$. Consequently, we would expect that the foreground switches domains while the background stays roughly the same. However, this could be problematic if the foregrounds do not share a similar shape (e.g. mapping a standing horse to a sitting zebra). To alleviate such issue we enforce that feature representations of $(1-A_Y(\hat{y}))\odot \hat{y}$ and $(1-A_X(x)) \odot x$ are similar via minimizing the feature matching loss:

% \begin{align}
%     L_{FM_{bg_x}} = \|f((1-A_Y(\hat{y}))\odot \hat{y}) - f((1-A_X(x)) \odot x)\|_1,
% \end{align}
% with $f$ being a feature extractor (e.g. resnet, inception net ...etc).

% Finally in order to make the mapping realistic we add an adversarial loss: 

% \begin{align}
%     L_{adv_x} = \E_{x \sim \Pr(x)}{log(D_X(x))} + \E_{x \sim \Pr(x), y \sim \Pr(y)}{log(1 - D_X(G_X(f_x,b_y)))}
% \end{align}

==> src/figs_cvpr/fig_giraffe.tex <==
\begin{figure*}[tb]
%Width of the figure

\centering
% \def\figheight{.2\linewidth}
%Sets the size of the table
\newcommand{\tableTitle}[1]{\scriptsize{#1}}%

%Default options for figures_cvpr
%\newlength{\imwidth}
%\setlength{\imwidth}{0.145\linewidth}
\setlength{\imwidth}{0.145\linewidth}
% \def\defaultops{width=0.16\columnwidth}%
% \renewcommand{\arraystretch}{0.8}%
\setlength{\tabcolsep}{0.3pt}%
%\renewcommand{\arraystretch}{1.5}
\setbox1=\hbox{\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_24_2.jpg}}%
\begin{tabular}{cccccc}

\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_24_2.jpg}\llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figgiraffe/imtemplate_25.jpg}}}}&
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/mask_4_1.jpg}&
% \llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figgiraffe/real_cropped_4.jpg}}}}&
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_24_3.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/mask_4_7.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_49_2.jpg}\llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figgiraffe/imtemplate_50.jpg}}}}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/mask_5_4.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_49_9.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_76_0.jpg}\llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figgiraffe/imtemplate_77.jpg}}}}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/mask_5_4.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/m_76_4.jpg}\\

%\rotatebox{90}{Our Final} &
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_25_2_0.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/rgb_4_1_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_25_3_0.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/rgb_4_7_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_50_2_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_50_9_1.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_77_0_3.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_77_4_0.jpg}\\

\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_25_2_4.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/rgb_4_1_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_25_3_4.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/rgb_4_7_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_50_2_2.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_50_9_2.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_77_0_2.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im_77_4_4.jpg}\\

\includegraphics[width=\imwidth]{figures/figgiraffe/child_final_63_0.jpg}&
% \includegraphics[width=\imwidth]{figures/figgiraffe/00004_predicted_image_canvas.jpg}&
\includegraphics[width=\imwidth]{figures/figgiraffe/child_final_63_6.jpg}&
\includegraphics[width=\imwidth]{figures/figgiraffe/child_final_68_0.jpg}&
\includegraphics[width=\imwidth]{figures/figgiraffe/child_final_68_1.jpg}&
\includegraphics[width=\imwidth]{figures/figgiraffe/child_final_91_0.jpg}&
\includegraphics[width=\imwidth]{figures/figgiraffe/child_final_91_6.jpg}\\

\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im1_m_24_2.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/rgb_4_1_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im1_m_24_3.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/rgb_4_7_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im3_m_49_2.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im3_m_49_9.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im2_m_76_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/im2_m_76_4.jpg}\\

    %  \tableTitle{Input Image} & %
%\vspace*{\fill}{\rotatebox[origin=c]{90}{~\cite{HierarchicalSemanticImageManpulation}}}\vspace*{\fill}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00004_predicted_image_canvas.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00004_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00004_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00009_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00009_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00024_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00024_predicted_image_canvas.jpg}\\

%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/child_final_63_0.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/00004_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/child_final_63_6.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/child_final_68_0.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/child_final_68_1.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/child_final_91_0.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figgiraffe/child_final_91_6.jpg}\\
    %  \tableTitle{Input Image} & %
    %  \tableTitle{Input Mask} & %
    % \tableTitle{InstaGAN Output}& %
    % \tableTitle{Our Output} & %
    % \tableTitle{InstaGAN Mask} & %
    % \tableTitle{Our Mask} %
 \end{tabular}
 
  \caption{COCO class \emph{Giraffe}. \emph{First row:} Our multiple generated masks conditioned on the background image given the bounding box. \emph{Second-Third row:} Our textured results. \emph{Fourth row:} Deterministic image generation by Hong et al.'s algorithm~\cite{HierarchicalSemanticImageManpulation}. \emph{Fifth row:} FineGAN's whole-image generation~\cite{finegan}. \emph{Last row:} Copy and Paste + deep harmonization baselines.
  }
 \label{fig:giraffe}
\vspace{-0.25cm}
\end{figure*}

==> src/figs_cvpr/fig_zebra.tex <==
\begin{figure*}[tb]
%Width of the figure

\centering
% \def\figheight{.2\linewidth}
%Sets the size of the table
\newcommand{\tableTitle}[1]{\scriptsize{#1}}%

%Default options for figures_cvpr
%\newlength{\imwidth}
%\setlength{\imwidth}{0.145\linewidth}
\setlength{\imwidth}{0.145\linewidth}
% \def\defaultops{width=0.16\columnwidth}%
% \renewcommand{\arraystretch}{0.8}%
\setlength{\tabcolsep}{0.3pt}%
%\renewcommand{\arraystretch}{1.5}
\setbox1=\hbox{\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_4_0.jpg}}%
\begin{tabular}{cccccc}

\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_4_0.jpg}\llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figzebra/imtemplate_5.jpg}}}}&
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/mask_4_1.jpg}&
% \llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figzebra/real_cropped_4.jpg}}}}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_4_5.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/mask_4_7.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_43_0.jpg}\llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figzebra/imtemplate_44.jpg}}}}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/mask_5_4.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_43_2.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_22_0.jpg}\llap{\makebox[\wd1][l]{\raisebox{0.5\imwidth}{\includegraphics[cfbox=white,width=0.5\imwidth]{figures_cvpr/figzebra/imtemplate_23.jpg}}}}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/mask_5_4.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/m_22_9.jpg}\\

%\rotatebox{90}{Our Final} &
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_5_0_0.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/rgb_4_1_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_5_5_0.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/rgb_4_7_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_44_0_3.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_44_2_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_23_0_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_23_9_0.jpg}\\

\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_5_0_4.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/rgb_4_1_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_5_5_2.jpg}& 
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/rgb_4_7_0.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_44_0_1.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_44_2_3.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_23_0_2.jpg}& 
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im_23_9_2.jpg}\\

\includegraphics[width=\imwidth]{figures/figzebra/child_final_0_0.jpg}&
\includegraphics[width=\imwidth]{figures/figzebra/child_final_0_1.jpg}&
\includegraphics[width=\imwidth]{figures/figzebra/child_final_0_2.jpg}&
\includegraphics[width=\imwidth]{figures/figzebra/child_final_0_3.jpg}&
\includegraphics[width=\imwidth]{figures/figzebra/child_final_0_4.jpg}&
\includegraphics[width=\imwidth]{figures/figzebra/child_final_0_5.jpg}\\

\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im1_m_4_0.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im1_m_4_5.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im3_m_43_0.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im3_m_43_2.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im2_m_22_0.jpg}&
\includegraphics[width=\imwidth]{figures_cvpr/figzebra/im2_m_22_9.jpg}\\
%\vspace*{\fill}{\rotatebox[origin=c]{90}{~\cite{HierarchicalSemanticImageManpulation}}}\vspace*{\fill}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/00004_predicted_image_canvas.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/00004_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/00004_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/00009_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/00009_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/00024_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/00024_predicted_image_canvas.jpg}\\

%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/child_final_63_0.jpg}&
% \includegraphics[width=\imwidth]{figures_cvpr/figzebra/00004_predicted_image_canvas.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/child_final_63_6.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/child_final_68_0.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/child_final_68_1.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/child_final_91_0.jpg}&
%\includegraphics[width=\imwidth]{figures_cvpr/figzebra/child_final_91_6.jpg}\\
    %  \tableTitle{Input Image} & %
    %  \tableTitle{Input Mask} & %
    % \tableTitle{InstaGAN Output}& %
    % \tableTitle{Our Output} & %
    % \tableTitle{InstaGAN Mask} & %
    % \tableTitle{Our Mask} %
 \end{tabular}
 
  \caption{COCO class \emph{Zebra}. \emph{First row:} Our multiple generated masks conditioned on the background image given the bounding box. \emph{Second-Third row:} Our textured results. \emph{Fourth row:} Deterministic image generation by Hong et al.'s algorithm~\cite{HierarchicalSemanticImageManpulation}. \emph{Fifth row:} FineGAN's whole-image generation~\cite{finegan}. \emph{Last row:} Copy and Paste + deep harmonization baselines. \ym{We should say somewhere that zebra texture results are less diverse}
  }
 \label{fig:giraffe}
\vspace{-0.25cm}
\end{figure*}

==> src/includes.tex <==
\usepackage{enumitem}
\usepackage{url}
\usepackage{amsthm}
\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{pbox}
\usepackage[utf8]{inputenc}
\usepackage{mathtools}
%\usepackage[nameinlink]{cleveref}
\usepackage[export]{adjustbox} 
\usepackage{longtable}
\usepackage{rotating}
\usepackage{adjustbox}

\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{url}
\usepackage{amsthm}
\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{pbox}
\usepackage[utf8]{inputenc}
\usepackage{mathtools}
%\usepackage[nameinlink]{cleveref}
\usepackage[export]{adjustbox} 
\usepackage{longtable}
\usepackage{rotating}
\usepackage{adjustbox}
\usepackage[shortlabels]{enumitem}
\usepackage{array}
\usepackage{makecell}
\usepackage{graphicx}
\usepackage{graphbox} %loads graphicx package


% \DeclareMathOperator{\E}{\mathbb{E}}
% \usepackage{import}
% \usepackage{tikz}
% \usepackage{extarrows}
% \usepackage{xparse} % For calculating aspect ratio
% \usepackage{calc} % For calculations
% %\usepackage{todonotes}
% \usepackage[moderate,mathdisplays=normal,wordspacing=normal]{savetrees}
\usepackage{colortbl}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{tablefootnote}
\usepackage{tabularx}
\usepackage{standalone}

%\setlength{\parskip}{.8em}

\definecolor{rowblue}{RGB}{220,230,240}
\definecolor{Orange}{RGB}{255,204,153}
\definecolor{Blue}{RGB}{153,204,255}
%%% From https://tex.stackexchange.com/questions/1522/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink.
%href fix
%\usepackage{etoolbox}
%\captionsetup{compatibility=false}


\DeclareMathOperator{\E}{\mathbb{E}}
\usepackage{import}
\usepackage{tikz}
\usepackage{extarrows}
\usepackage{xparse} % For calculating aspect ratio
\usepackage{calc} % For calculations
%\usepackage{todonotes}
% \usepackage[moderate,mathdisplays=normal,wordspacing=normal]{savetrees}
\usepackage{colortbl}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{tablefootnote}
\usepackage{tabularx}
\usepackage{standalone}
\definecolor{rowblue}{RGB}{220,230,240}
\definecolor{Orange}{RGB}{255,204,153}
\definecolor{Blue}{RGB}{153,204,255}

\usepackage{arydshln}


%%% From https://tex.stackexchange.com/questions/1522/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink.
%href fix
\usepackage{etoolbox}
\makeatletter
\patchcmd\@combinedblfloats{\box\@outputbox}{\unvbox\@outputbox}{}{\errmessage{\noexpand patch failed}}
\makeatother
%%%

%Macro to expand options for Graphics
\makeatletter
\define@key{Gin}{expandoptions}{%
  \begingroup
  \edef\x{\endgroup
    \noexpand\setkeys{Gin}{#1}%
  }\x
}
\makeatother

%Debug later
%Shadowing for Image Graphics

% % %Add shadow to image:
% \usetikzlibrary{shadows,calc}%

% % code adapted from https://tex.stackexchange.com/a/11483/3954

% % some parameters for customization
% \def\shadowshift{0.5pt,-0.5pt}%
% \def\shadowradius{1pt}%

% \colorlet{innercolor}{black!60}%
% \colorlet{outercolor}{gray!05}%

% % this draws a shadow under a rectangle node
% \newcommand\drawshadow[1]{
%     \begin{pgfonlayer}{shadow}
%         \shade[outercolor,inner color=innercolor,outer color=outercolor] ($(#1.south west)+(\shadowshift)+(\shadowradius/2,\shadowradius/2)$) circle (\shadowradius);
%         \shade[outercolor,inner color=innercolor,outer color=outercolor] ($(#1.north west)+(\shadowshift)+(\shadowradius/2,-\shadowradius/2)$) circle (\shadowradius);
%         \shade[outercolor,inner color=innercolor,outer color=outercolor] ($(#1.south east)+(\shadowshift)+(-\shadowradius/2,\shadowradius/2)$) circle (\shadowradius);
%         \shade[outercolor,inner color=innercolor,outer color=outercolor] ($(#1.north east)+(\shadowshift)+(-\shadowradius/2,-\shadowradius/2)$) circle (\shadowradius);
%         \shade[top color=innercolor,bottom color=outercolor] ($(#1.south west)+(\shadowshift)+(\shadowradius/2,-\shadowradius/2)$) rectangle ($(#1.south east)+(\shadowshift)+(-\shadowradius/2,\shadowradius/2)$);
%         \shade[left color=innercolor,right color=outercolor] ($(#1.south east)+(\shadowshift)+(-\shadowradius/2,\shadowradius/2)$) rectangle ($(#1.north east)+(\shadowshift)+(\shadowradius/2,-\shadowradius/2)$);
%         \shade[bottom color=innercolor,top color=outercolor] ($(#1.north west)+(\shadowshift)+(\shadowradius/2,-\shadowradius/2)$) rectangle ($(#1.north east)+(\shadowshift)+(-\shadowradius/2,\shadowradius/2)$);
%         \shade[outercolor,right color=innercolor,left color=outercolor] ($(#1.south west)+(\shadowshift)+(-\shadowradius/2,\shadowradius/2)$) rectangle ($(#1.north west)+(\shadowshift)+(\shadowradius/2,-\shadowradius/2)$);
%         \filldraw ($(#1.south west)+(\shadowshift)+(\shadowradius/2,\shadowradius/2)$) rectangle ($(#1.north east)+(\shadowshift)-(\shadowradius/2,\shadowradius/2)$);
%     \end{pgfonlayer}
% }

% \usetikzlibrary{backgrounds}%

% % create a shadow layer, so that we don't need to worry about overdrawing other things
% \pgfdeclarelayer{shadow}%
% \pgfsetlayers{shadow,main}%


% \newcommand\shadowimage[2][]{%
% \begin{tikzpicture}%
% \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[#1]{#2}};
% \drawshadow{image}%
% \end{tikzpicture}}%
% %END AD SHADOW TO IMAGE

%Calculates the aspect ratio of an image
\ExplSyntaxOn
\NewDocumentCommand{\aspectratio}{smo}
 {% #2 is the image file
  \hbox_set:Nn \l_tmpa_box {\includegraphics{#2}}
  \IfNoValueTF{#3}
   {
    \__student_aspectratio:nn { \box_wd:N \l_tmpa_box } { \box_ht:N \l_tmpa_box }
   }
   {
    \IfBooleanTF{#1}{ \tl_gset:Nx } { \tl_set:Nx } #3
     {
      \__student_aspectratio:nn { \box_wd:N \l_tmpa_box } { \box_ht:N \l_tmpa_box }
     }
   }
 }

%Ignore this error; the Latex function works
% \cs_new:Nn \__student_aspectratio:nn
%  {
%   \fp_eval:n {round( #1 / #2 , 5)}
%  }
% \ExplSyntaxOff


\newcommand{\ow}[1]{\textbf{\textcolor[rgb]{.1, .6, .1}{OW: #1}}}%
\newcommand{\jt}[1]{\textbf{\textcolor[rgb]{.8, .1, .1}{JT: #1}}}%
\newcommand{\ag}[1]{\textbf{\textcolor[rgb]{.1, .1, .8}{AG: #1}}}%
\newcommand{\ym}[1]{\textbf{\textcolor[rgb]{.8, .1, .8}{YM: #1}}}%
\newcommand{\kimki}[1]{\textbf{\textcolor[rgb]{.1, .8, .8}{KK: #1}}}%
\newcommand{\todo}[1]{\textbf{\textcolor[rgb]{.8, .1, .1}{#1}}}%

\newcommand{\tableDir}{src/tables/}%
\newcommand{\figDir}{src/figures/}%

\newcommand{\calL}{\mathcal{L}}

%Save default lengths
\newlength{\mytabcolsep}%
\setlength{\mytabcolsep}{\tabcolsep}%
\let\myarraystretch\arraystretch%

\def\I{\mathcal{I}}
\def\T{\mathcal{T}}
\def\S{\mathcal{S}}
\def\D{\mathcal{D}}
\def\p{\mathbf{p}}
% \def\t{\mathbf{t}}
\def\R{\mathbf{R}}
\def\w{\mathbf{\omega}}
\def\x{\mathbf{x}}
\def\W{\mathcal{W}}
\def\L{\mathcal{L}}
\def\m{\mathbf{m}}
\def\M{\mathbf{M}}
\def\s{\mathbf{s}}
\def\t{\mathbf{t}}
% \def\t{\mathbf{t}}

\newcommand{\model}{Proposed}


==> src/tables/tabKID.tex <==
\begin{table}[t]
%Width of the figure
\centering%
\caption{%
Kernel Inception Distance$\times 100 \pm \text{std} \times 100$ across all datasets used. Lower is better. \kimki{(highlighted in boldface)}}
\label{tab:KID1}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{lrrrr}
\toprule
Models & \emph{Giraffe} & \emph{Zebra} & \emph{Pizza} & \emph{Bus} \\
\midrule
SIM~\cite{HierarchicalSemanticImageManpulation} & 11.74 $\pm$ 0.77 & 14.39 $\pm$ 1.23 & 16.24 $\pm$ 0.84 & 5.60 $\pm$ 0.44\\
Ours & \textbf{7.59 $\pm$ 0.63} & \textbf{2.57 $\pm$ 0.17} & \textbf{14.76 $\pm$ 0.85} & \textbf{2.93 $\pm$ 0.33} \\
\midrule
FineGan~\cite{finegan} &13.98 $\pm$ 1.17 & 7.06 $\pm$ 0.93 & 8.13 $\pm$ 1.20 & 7.03 $\pm$ 0.85\\
Ours & \textbf{4.79 $\pm$ 0.66} & \textbf{5.02 $\pm$ 1.11} & \textbf{5.96 $\pm$ 0.68} & \textbf{3.41 $\pm$ 0.65}\\
\bottomrule
\end{tabular}
}
\vspace{-0.4cm}
\end{table}

==> src/tables/tableKID_rebuttal.tex <==
\begin{table}[t]
%Width of the figure
\centering%
\caption{%
Kernel Inception Distance$\times 100 \pm \text{std} \times 100$. Lower is better.}
\label{tab:KID1}
\begin{tabular}{lrrrr}
\toprule
Models & \emph{Giraffe} & \emph{Zebra}\\
\midrule
cut and paste & \textbf{5.47 $\pm$ 0.54} & 2.66 $\pm$ 0.27 \\
Ours & 7.59 $\pm$ 0.63 & \textbf{2.57 $\pm$ 0.17} \\
\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table}
